Annotation-efficient cancer detection with report-guided lesion annotation for deep learning-based prostate cancer detection in bpMRI

Deep learning-based diagnostic performance increases with more annotated data, but large-scale manual annotations are expensive and labour-intensive. Experts evaluate diagnostic images during clinical routine, and write their findings in reports. Leveraging unlabelled exams paired with clinical reports could overcome the manual labelling bottleneck. We hypothesise that detection models can be trained semi-supervised with automatic annotations generated using model predictions, guided by sparse information from clinical reports. To demonstrate efficacy, we train clinically significant prostate cancer (csPCa) segmentation models, where automatic annotations are guided by the number of clinically significant findings in the radiology reports. We included 7,756 prostate MRI examinations, of which 3,050 were manually annotated. We evaluated prostate cancer detection performance on 300 exams from an external centre with histopathology-confirmed ground truth. Semi-supervised training improved patient-based diagnostic area under the receiver operating characteristic curve from $87.2 \pm 0.8\%$ to $89.4 \pm 1.0\%$ ($P<10^{-4}$) and improved lesion-based sensitivity at one false positive per case from $76.4 \pm 3.8\%$ to $83.6 \pm 2.3\%$ ($P<10^{-4}$). Semi-supervised training was 14$\times$ more annotation-efficient for case-based performance and 6$\times$ more annotation-efficient for lesion-based performance. This improved performance demonstrates the feasibility of our training procedure. Source code is publicly available at github.com/DIAGNijmegen/Report-Guided-Annotation. Best csPCa detection algorithm is available at grand-challenge.org/algorithms/bpmri-cspca-detection-report-guided-annotations/.

==> appendices/a-STARD.tex <==
\subsection{STARD diagram}
\blue{PENDING}. 

==> appendices/appendices.tex <==
\newpage
\appendix
\renewcommand{\theHfigure}{Appendix.\thetable}
\renewcommand\thefigure{\thesubsection.\arabic{figure}}

\setcounter{figure}{0} % prepend to each appendix
% \input{appendices/a-STARD}
\input{appendices/b-detection-model}
% \input{appendices/c-augmentation-overview}
\input{appendices/d-AVA-quality-DSC}

==> appendices/b-detection-model.tex <==
\subsection{Detection Model Architecture}
\label{sec:detection_model_architectures}
For our prostate cancer segmentation task, \namennUNet\ configured itself to use a 3D \nameUNet\ with five down-sampling steps, as shown in \Cref{fig:detector_networks}. This figure also shows the specific choice of 2D/3D convolutional blocks, max-pooling layers and transposed convolutions. % is best conveyed based on the figure.  
No cascade of \nameUNets\ or 2D \nameUNet\ was triggered for our dataset. 

% Specifically, the anisotropic \nameUNet\ has two down-sampling steps where the pooling and convolutions happen in 2D, followed by two down-sampling steps where both pooling and convolutions happen in 3D, and finally one down-sampling step with pooling in 2D and convolutions in 3D. Each convolutional block contains two convolutional layers with kernel size $1\times 3\times 3$ in 2D and kernel size $3\times 3\times 3$ in 3D. 
% No cascade of \nameUNets\ or 2D \nameUNet\ was triggered for our dataset. 

The implementation of the \nameUNetagpp\ architecture is the same as in \citep{saha2021end}, with the exception of \nameLeakyReLU\ \citep{maas2013rectifier} activations throughout the decoder and decreased $L_2$ kernel regularisation of $10^{-4}$. See \citep{saha2021end} for implementation details. 

\input{figures/detector_networks}


==> appendices/c-augmentation-overview.tex <==
\subsection{Augmentations}
\input{chapters/deprecated/2f-augmentation-details}

==> appendices/d-AVA-quality-DSC.tex <==

\input{figures/AVA-quality-DSC}

==> appendices/thesis-appendices.tex <==
\newpage
\appendix
\input{appendices/thesis/a-rician-noise}
\input{appendices/thesis/b-data}
\input{appendices/thesis/c-active-surveillance}
\input{appendices/thesis/d-image-registration}
\input{appendices/thesis/e-dynamic-threshold-pipeline}



==> appendices/thesis/a-rician-noise.tex <==
\subsection{Rician noise}
% introduce data augmentations
Data augmentation is one of the most import techniques to improve the generalisation of deep learning models to unseen data. Typical data augmentations include rotation, mirroring, translation and zooming, but many more exist. When training a network with data augmentations, the training samples are transformed with one or multiple augmentations before being provided to the network. As a result, the network is guided to make its predictions invariant under these transformations, which results in a model that generalises better to unseen data. 

% introduce intensity based augmentations
At the start of my internship, the group's data augmentation pipeline consisted of rotation, translation, horizontal flipping and zooming, which are all geometric transformations. To improve the data augmentation pipeline, I have investigated intensity based augmentations, which are complementary to geometric transformations. While geometric transformations move the original voxels around in some structured way, intensity based augmentations preserve the location of the voxels and apply noise to each voxel. 

% introduce Rician noise
Intensity based augmentations span a large domain of additive, multiplicative and/or any nonlinear function based on the original voxel value. %  and/or multiplicative noise, with noise parameters drawn from any distribution. 
One of the best known intensity based augmentations is additive Gaussian noise, where noise following the Gaussian distribution is added to each voxel individually:
\begin{equation}
    I_{new} = I_{old} + \mathcal{N}(0, \sigma^2)
\end{equation}
Where $\mathcal{N}$ is the Gaussian distribution and $\sigma^2$ the variance. 

A drawback of additive Gaussian noise is that the intensities can become negative, which is physically impossible for MRI sequences such as T2W and DWI (these scans as used by radiologists and this work are magnitude maps; phase maps can be negative, but are typically disregarded). Noise in MRI scans is shown to be governed by the Rician distribution \citep{gudbjartsson1995rician}, which is non-negative and approaches the Gaussian distribution for large values. The Rician distribution is given by:
\begin{equation}
    I_{new} = \sqrt{(I_{old} + \sigma \cdot \phi)^2 + (\sigma\cdot\phi)2}
\end{equation}
Where $\sigma$ is the magnitude of the Rician distribution and $\phi$ is drawn from $\mathcal{N}(0, 1)$ for each voxel individually. 


% \newcommand\footnoteMisalignment{\footnote{When opened in ITK-SNAP, the scans would appear properly aligned. However, for some cases the centres of the fields of view were different. This was not accounted for, resulting in a misalignment of more than 2 mm after preprocessing for \numVisitsMisalignedExcluded\ ($1.6\%$). Properly accounting for the difference in centres proved difficult, so I adapted the pipeline to exclude these cases which would be misaligned otherwise. }}
\newcommand\footnoteMisalignment{\footnote{Accounting for the misalignment proved difficult, so I excluded \numVisitsMisalignedExcluded\ cases ($1.6\%$) which otherwise would have a misalignment of at least 2 mm. }}

% introduce dynamic preprocessing pipeline
Motivated by the physical relevance of the Rician distribution, I have adapted the data pipeline to incorporate this distribution as data augmentation. This required an overhaul of the way the scans are preprocessed, because the Rician noise needs to be applied at native resolution and initially the scans were resampled at an early stage. The new preprocessing pipeline saves the scans at original resolution, and resamples them on-the-fly during model training, after applying the Rician noise data augmentation. This overhaul also resulted in a good understanding of the preprocessing steps, which led to the discovery of a bug where T2W and ADC/DWI scans became misaligned due to the preprocessing pipeline\footnoteMisalignment.

% introduce experiment
To determine a good magnitude for the Rician noise ($\sigma$), I identified the range of $\sigma \in [0, 0.05]$ as relevant values through visual inspection, and tested $\sigma=0.00$, $0.01$, $0.02$, $0.03$, $0.04$ and $0.05$. During training, the Rician noise is applied with a probability of $75\%$. For each magnitude, models were trained with 5-fold cross-validation and 2 restarts. The resulting 10 performance metrics were compared using the permutation test with \numIterationsPermutationTest\ iterations. To retain the integrity of the external test set (ZGT), each model is evaluated on the RUMC dataset. 

% results
To evaluate the patient based diagnostic performance we can leverage the \numUnlabelledStudiesFullDataset\ unlabelled RUMC visits, which results in a much more stable evaluation compared to the $\approx 300$ labelled studies in each validation fold\footnote{This number is lower than 1/5th of all labelled samples, because samples with positive MRI (PI-RADS $\geq 3$) but unknown biopsy result were excluded from the validation set. }. For these unlabelled visits the ground truth is derived by automatically extracting the scores from pathology and radiology reports. To construct labels with low error rate and typical distribution of low-, intermediate and high risk patients, a method similar to ProstateX was employed: cases with Gleason grade group $\geq 2$ are positive and cases with either Gleason grade group $\leq 1$ or PI-RADS $\leq 2$ are negative. This gives 883 biopsy-confirmed positive cases and 2,656 negative cases. 

The patient based diagnostic performances as evaluated against the ProstateX-like labels are given in \Cref{fig:rician-noise-AUC-performance}. The statistical significance p-values are given in \Cref{fig:rician-noise-AUC-significance-matrix}. Small amounts of Rician noise ($\sigma \in [0.01, 0.03]$) as data augmentation may improve patient based model performance, but not with statistical significance ($P = 0.17-0.55$). 
\input{figures/rician-noise-AUC-performance}
\input{figures/rician-noise-AUC-significance-matrix}

To evaluate lesion based diagnostic performance, manually annotated cases are required. The 5-fold cross-validation results in five validation sets with small differences in difficulty, resulting is slightly higher or lower performance metrics across all models for some validation folds. Differences in model performance can be highlighted by accounting for this variation intrinsic to the data, by shifting the metrics by a single constant per fold. In \Cref{fig:rician-noise-pAUC-three} the unmodified partial Area Under the Free-Response Operating Characteristic curve (pAUC) values are shown in the \ieeeblue{left}\ panel, the pAUC values shifted per fold by the mean pAUC of the baseline ($\sigma = 0$) are shown in the \ieeeblue{middle}\ panel and the statistical significance p-values between the different Rician noise magnitudes are shown in the \ieeeblue{right}\ panel. Small amounts of Rician noise ($\sigma \in [0.01, 0.03]$) as data augmentation may improve lesion based model performance, but not with statistical significance ($P = 0.07-0.28$). 

\input{figures/rician-noise-pAUC-three}

% conclusion
The experiments suggest that Rician noise as data augmentation may improve both patient based and lesion based diagnostic performance, but neither metric improved with statistical significance. Based on prior experience from Kaggle challenges, I believe that intensity based data augmentations should be part of any data augmentation pipeline by default, and only taken out if motivated by experiments, rather than the other way around. This is also motivated by the data augmentation pipeline from the \namennUNet\ framework, which employs additive Gaussian noise, brightness, contrast and gamma augmentations as intensity based data augmentations for all datasets. While Rician noise at native resolution (before resampling the MRI sequences to a shared voxel spacing) is well suited for MRI in theory, the experiments in this appendix do not warrant rewriting a preprocessing pipeline to incorporate this specific augmentation. Instead of incorporating this single augmentation, it is probably more beneficial to adopt the data augmentation pipeline from \namennUNet, which has the standard geometric transformations, four intensity based augmentations, Gaussian blur and simulation of low resolution, all with magnitudes and probabilities backed by large-scale experiments. 

==> appendices/thesis/b-data.tex <==
\subsection{Data}
%%%%%%%%%%%%%%%%%%
%% Introduction %%
%%%%%%%%%%%%%%%%%%
This appendix gives an overview of several data related projects during my internship. The aim of these projects was to improve the prostate MRI archive, annotations, metadata and study selection, and the goal of this appendix is to describe the changes made throughout the year and to provide documentation to future researchers. 

% intro section 1
The first section, \Cref{sec:preprocessing-RUMC-visits}, describes changes made to the preprocessing pipeline from DICOM archive to MHA scans. This section also highlights some of the design choices, to facilitate future improvements to the pipeline. 

% intro section 2
The second section, \Cref{sec:improving-RUMC-annotations}, describes improvements to the radiology based annotations of the RUMC dataset. This section also highlights efforts to improve the longevity of the annotation archive. 

% intro section 3
The third section, \Cref{sec:extracting-RUMC-metadata}, describes the extraction of Gleason scores from pathology reports, extraction of measurements from the radiology reports (prostate volume, PSA and PSA density) and extraction of prior Gleason scores and treatment from the radiology reports. 

% intro section 4
The fourth section, \Cref{sec:exclusion-criteria-RUMC}, describes the exclusion criteria employed for the RUMC dataset. This section also highlights the transparent pipeline for exclusion criteria. 

% intro section 5
The fifth and final section, \Cref{sec:preprocessing-UMCG-dataset}, describes the preparation of the UMCG dataset. Specifically, the naming scheme, study selection and naming errors are highlighted. 

%%%%%%%%%%%%%%%%%
%% RUMC images %%
%%%%%%%%%%%%%%%%%
\newcommand\seriesDescription{\texttt{series description}}
\newcommand\exampleSeriesDescriptionADC{\texttt{ep2d\_diff\_tra\_ADC\_DFC}}
\newcommand\exampleSeriesDescriptionTtwoW{\texttt{t2\_tse\_tra}}

\subsubsection{Preprocessing RUMC prostate MRI visits}
\label{sec:preprocessing-RUMC-visits}
The preprocessing pipeline from DICOM archive to MHA scans selects the relevant MRI sequences and combines the individual DICOM slices to a single MHA file per MRI sequence. The pipeline is configured to convert the axial T2-weighted (T2W), diffusion weighted (DWI), apparent diffusion coefficient (ADC), sagittal T2W and coronal T2W scans. 

% study selection
% Approach to select DICOM series:
% 1. Select the DICOM series which match the user-defined tags (per modality) and retain the series matching 
%   the DICOM series description with highest priority (first in list)
% 2. If multiple series matched, retain the series with the most slices (and at least min_num_slices slices). 
%   Note: this will NOT select a scan with isotropic voxel spacing (e.g., t2_spc_3D_cor_iso) over an anisotropic 
%   scan (e.g., t2_tse_cor), as the anisotropic tag has higher priority (in this example).
% 3. If multiple series matched, and have the same number of slices, select the DICOM series with the highest in-plane resolution.
% 4. If the above tie-breakers are insufficient, select the first one (possibly quasi-random due to side-effects)

MRI sequences in the DICOM archive are described by their \seriesDescription, which are tags that describe the sequence in a semi-structured manner. Common examples are \exampleSeriesDescriptionTtwoW\ for axial T2W and \exampleSeriesDescriptionADC\ for axial ADC scans, with 9214 and 8748 occurrences, respectively. In total, there are 1585 different \seriesDescription s, of which most have low frequency and/or refer to a T1-weighted sequence for dynamic contrast enhanced imaging. To determine which tags should be used, I visually inspected scans from various tags with high prevalence together with Matin. This resulted in the series descriptions shown in \Cref{tab:MRI-sequences}. 

In an ideal world, these \seriesDescription s would be sufficient to select the correct MRI sequence, but about 1/4th of the studies have multiple MRI sequences with the same \seriesDescription. This seemed to be mainly caused by download issues from the Picture Archiving and Communication System (PACS) to our storage system, where one series would be incomplete (missing DICOM slices) and the other complete. To account for the presence of both complete and incomplete series, I selected the series with most slices (within the same \seriesDescription). When multiple series have the same \seriesDescription\ and the same number of slices, I select the series with the highest in-plane resolution. 

The tags shown in \Cref{tab:MRI-sequences} and the sequence selection steps described above resulted in 9099 studies with axial T2W, ADC, DWI, sagittal T2W and coronal T2W scan between 2014 and 2020. 

Code for the improved preprocessing pipeline can be found \href{https://github.com/DIAGNijmegen/AbdomenMRUS-pca-surveillance/blob/dfd889da23d2cfb3a60e0fbe476f44399c1378ee/Environment/Dicom2MHD/dicom_archive.py}{\underline{here}} and \href{https://github.com/DIAGNijmegen/AbdomenMRUS-pca-surveillance/blob/dfd889da23d2cfb3a60e0fbe476f44399c1378ee/Preprocessing/Convert-DICOM-archive.ipynb}{\underline{here}}  (requires DIAG access). My contributions: 
\begin{itemize}
    \item Identified additional \seriesDescription s
    \item Sped up pipeline $16\times$, reducing total preprocessing time from approx. 8 days to approx. 12 hours
    \item Wrote documentation for preprocessing pipeline
    \item Solved bug where scans became scrambled or blank
    \item Solved bug where the \seriesDescription s where matched incorrectly (affected approx. 50 scans) 
    \item Wrote verification of MHA archive (mainly to ensure studies are properly written to disk)
    \item Delivered MHA archive with approx. 5000 new visits
\end{itemize}

% 

\input{figures/MRI-sequences}

%%%%%%%%%%%%%%%%%%%%%%
%% RUMC annotations %%
%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Improving RUMC annotations}
\label{sec:improving-RUMC-annotations}
Annotations are one of the most important ingredients for training deep neural networks. During my internship I've worked on improving the annotations though combining different sources of information. Most notably, I've automatically split the majority of the PI-RADS $\geq 4$ annotations in separate PI-RADS 4 or 5 labels, and identified \percentageIncorrectAnnotationsIdentified\ cases with incorrect annotation (\percentageIncorrectAnnotationsIdentified\ of all annotations). 

Splitting the annotations in separate labels for PI-RADS 4 or 5 allows to train a machine learning model with improved risk-stratification, by assigning a higher risk to PI-RADS 5 than to PI-RADS 4. Split annotations also allow more fine-grained meta-analysis, and paved the way to also annotate the PI-RADS 3 lesions as a separate label. The automatic conversion script was able to confidently split 3,540/3,652 ($97\%$) cases, leaving 112 cases. These 112 remaining cases have been manually split by Ilse, meaning the annotation archive is now completely split into PI-RADS 4 and 5. 

% comment:22: Splitting csPCa annotations into PI-RADS 4 or 5
% comment:29: Dataset conversion

My contributions: 
\begin{itemize}
    \item Automatically split 3,540/3,652 ($97\%$) PI-RADS $\geq 4$ annotations in either PI-RADS 4 or 5
    \item Orchestrated several (small) annotation projects with Ilse 
    \item Set up GitHub archive for annotations, which makes adding and revising annotations transparent
    \item Identified \numIncorrectAnnotationsIdentified\ incorrect annotations (\percentageIncorrectAnnotationsIdentified\ of total). 
\end{itemize}


%% Corrected delineations %%
% See the overview in Development/2021-07-27-overview-revised-annotations

%%%%%%%%%%%%%%%%%%%
%% RUMC metadata %%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Extracting metadata from reports}
\label{sec:extracting-RUMC-metadata}
The dataset from RUMC is derived from clinical practice over the span of seven years, resulting in a lot of useful information, but not necessarily in a structured format. Reliable metadata for all studies is important for most downstream analyses, so during my internship I've set out to extract metadata from the radiology and pathology reports. The benefit of radiology and pathology reports is that those are available across all years, but the drawback is that reports are free form text. 

Apart from extracting PI-RADS scores from radiology reports, I've also extracted: 
\begin{itemize}
    \item Gleason scores and biopsy dates from pathology reports
    \item PSA level, PSA density, prostate volume, prior treatment and prior Gleason scores from radiology reports
\end{itemize}

The extraction method for this metadata is similar to the PI-RADS extraction described in \Cref{sec:automatic_finding_extraction}, albeit a bit simpler. Code can be found \href{https://github.com/DIAGNijmegen/AbdomenMRUS-pca-surveillance/blob/dfd889da23d2cfb3a60e0fbe476f44399c1378ee/Preprocessing/Enrich-Metadata.ipynb}{\underline{here}} (requires DIAG access). 

\input{figures/STARD-RUMC}
% comment:15
% comment:23
% comment:36: Automatic extraction of PI-RADS scores from radiology reports

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% RUMC exclusion criteria %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Exclusion criteria RUMC}
\label{sec:exclusion-criteria-RUMC}
Studies with treatment or a positive biopsy (Gleason score $\geq 3+4$) prior to the MRI scan are excluded, as well as studies with bad MRI scan quality and studies from patients who opted out. 
To identify studies with prior treatment, I started with the list of treatments used by Matin, and extended that list by looking for additional treatments in the radiology reports. 
The list of treatments can be found in \Cref{tab:excluded-treatments}. 
I also excluded follow-up studies, even if the subsequent report didn't repeat the prior treatment. 
The improved pipelin resulted in identifying an additional \additionalTreatmentsFound\ studies with prior treatment (\additionalTreatmentsFoundPercentage\ more). 

Further documentation, details and lists of excluded studies can be found \href{https://github.com/DIAGNijmegen/AbdomenMRUS-pca-surveillance/blob/dfd889da23d2cfb3a60e0fbe476f44399c1378ee/Environment/config/exclusion_criteria.py}{\underline{here}} (requires DIAG access). The STARD diagram showing the number of studies included and excluded in this work is shown in \Cref{fig:STARD-RUMC}. 
% comment:19
% comment:20
% comment:24: Exclusion criteria: prior treatment and image artifacts

\input{figures/table-treatments}

%%%%%%%%%%
%% UMCG %%
%%%%%%%%%%
\subsubsection{UMCG dataset}
\label{sec:preprocessing-UMCG-dataset}
The dataset from UMCG remained unused in my project, but I did prepare it. This involved collaborating with Jeroen and Christian to receive additional metadata, documentation and understanding their naming scheme. Furthermore, I extended the preprocessing pipeline described in \Cref{sec:preprocessing-RUMC-visits} to harmonise the datasets from UMCG and RUMC. The prepared dataset and documentation can be found at \verb!Chansey::pelvis/data/prostate-MRI/umcg/!. Code can be found \href{https://github.com/DIAGNijmegen/AbdomenMRUS-pca-surveillance/blob/dfd889da23d2cfb3a60e0fbe476f44399c1378ee/Preprocessing/Convert-RUMC-Annotations.ipynb}{\underline{here}} and \href{https://github.com/DIAGNijmegen/AbdomenMRUS-pca-surveillance/blob/dfd889da23d2cfb3a60e0fbe476f44399c1378ee/Preprocessing/Convert-UMCG-archive.ipynb}{\underline{here}} (requires DIAG access). 

Visits in our internal RUMC dataset are identified by a unique patient identifier and a unique study identifier. Using these two identifiers, it is straightforward to identify which studies belong to the same patient, and new visits can be added to the archive without affecting the naming scheme of existing visits. A similar naming scheme can be constructed for the UMCG dataset using their markdatasheet. 

\newcommand\patientID{\texttt{anon\_id}}
\newcommand\visitNum{\texttt{ret\_pat\_number}}
\newcommand\redcapID{\texttt{redcap\_id}}
\newcommand\studyID{\texttt{[redcap\_id]-[ret\_pat\_number]}}
Visits in the external UMCG dataset can be uniquely identified using the \redcapID\ (1 to 965) and \visitNum\ (empty for first visit, 1 for second visit and 2 for third visit), and patients can be uniquely identified using the \patientID\ (e.g., M-001 or U-001). To harmonise the naming scheme with the RUMC dataset, the \redcapID\ and \visitNum\ are combined to a unique study identifier as \studyID, where an empty \visitNum\ is replaced by a zero. 


% patient id: M-ddd or U-ddd, with ddd a three-digit number. 
% visit num: empty for first visit, 1 for second, 2 for third, ...
% redcap id: identifier for (a sequence of) visits of a patients

The UMCG dataset consists of MRI examinations from UMCG, Martini Ziekenhuis and peripheral hospitals throughout the province of Groningen. Studies from UMCG or Martini have \texttt{mri\_location\_1 == 1}, while studies from peripheral hospitals have \texttt{mri\_location\_1 == 2}, with the specific peripheral hospital described in \texttt{mri\_location\_2}. Studies from peripheral hospitals have large variance in acquisition parameters, so only including studies from UMCG or Martini may be recommended. 

Further study selection criteria are prior treatment, prior positive biopsies and bad scan quality. 
Prior treatment was an exclusion criteria for the UMCG dataset, so none of the studies we received should have prior treatment. Bad scan quality wasn't an explicit exclusion criterion, but scans that are of insufficient quality for interpretation are usually repeated, and if all went well we only received good scans. To exclude studies with previously confirmed prostate cancer we received an updated markdatasheet, with prior Gleason scores described in \texttt{prev\_tar\_gleas1}, \texttt{prev\_tar\_gleas2}, \texttt{prev\_trus\_g1} and \texttt{prev\_trus\_g2}. 

Although the UMCG dataset is of very high quality, it did contain several naming inconsistencies in its files, likely caused by manual typing errors. To resolve these inconsistencies in a transparent manner, Anindo and I created a \href{https://github.com/DIAGNijmegen/prostateMR_archive_umcg}{\underline{repository}} for the annotations and corrected the typing mistakes. 


==> appendices/thesis/c-active-surveillance.tex <==
\subsection{Active Surveillance}
Active Surveillance within prostate cancer management is an interesting and important direction to improve patient care. Working on deep learning solutions for Active Surveillance patients has taught me a lot, but did not result in concrete results. This lack of results was mainly caused by insufficient clinical motivation for the desired outcome. While existing Active Surveillance programs have shown excellent low prostate cancer mortality \citep{welty2015extended, selvadurai2013medium, klotz2015long, tosoian2015intermediate, bokhorst2016decade}, it is still relatively new. As a result, there is no clear target objective that a deep learning solution should aim for. 

Several options for target objectives exist: 
\begin{enumerate}
    \item Progression from Gleason grade group $\leq 1$ to Gleason grade group $\geq 2$
    \item Progression of PI-RADS score
    \item Identify new or vanished lesions
    \item Change of mean/min/std. ADC values within lesion mask
    \item Progression of lesion volume
\end{enumerate}

Unfortunately, all targets have limitations. Only few patients undergo multiple biopsies (1); PI-RADS scores suffer from large inter- and intra-reader variability, which is amplify when deriving change (2 \& 3); contours of lesions are often ill-defined, resulting in unstable statistics and volume (4 \& 5). 

The interested reader is encouraged to contact me (\href{mailto:Joeran.Bosma@radboudumc.nl}{Joeran.Bosma@radboudumc.nl}) for further discussions about Active Surveillance within prostate cancer management, and/or read the literature review I wrote on the deep learning side of it (\href{https://bosma.co/Bosma2021deep.pdf}{bosma.co/Bosma2021deep.pdf}. 

% Literature review: bosma.co/Bosma2021deep.pdf


==> appendices/thesis/d-image-registration.tex <==
\subsection{Image registration}
Image registration is a technique that can align medical scans that are similar but not exactly the same, which can be extremely helpful for a baseline and follow-up scan. 
An example is shown in \Cref{fig:registration-example}, where the first and third panel show the baseline and follow-up visits, and the second panel shows the baseline scan aligned to the follow-up scan. To align the baseline scan, it is moved `up' (towards anterior) and `pulled out of the page' (towards base), resulting in an aligned prostate. 

During my investigation of image registration for prostate MRI, I learned three practical lessons which I'd like to share:
\begin{enumerate}
    \item Normalise your scans before registration. Similar to deep learning, an image registration algorithm uses gradient ascent to optimise a similarity metric, and a registration can completely fail if those gradients are e.g. 1000 times higher than expected. 
    \item Registering the prostate segmentation masks, rather than the original scans, gives the most robust registration. A fine-grained registration of the original scans can then be compared to the robust registration, to spot cases where the fine-grained registration completely failed. 
    \item The structural similarity index metric (SSIM) is the metric that corresponds best with the true displacement, as shown by my brother \citep{bosma2021quantitative}. 
\end{enumerate}

% Image registration is difficult to quantitatively evaluate, 
% When I was working on Active Surveillance within prostate cancer diagnosis, I investigated image registration

\input{figures/registration-example}

==> appendices/thesis/e-dynamic-threshold-pipeline.tex <==
\subsection{Dynamic candidate extraction from softmax predictions}
When I started my internship, the method to extract lesion candidates from a model's softmax prediction involved a static threshold. Below this threshold, all model predictions were set to zero, and the remaining `islands' would then be the lesion candidates. This threshold was static across all samples, even though different models and even different datasets have different optimal thresholds. Other than tuning the static threshold for each model and dataset, there was no way to deduce a proper threshold. 

To circumvent the limitation of a static candidate extraction, I proposed a sample-dependent `dynamic' candidate extraction. This candidate extraction pipeline should extract `blobs' from the softmax prediction in a scale-free manner. The method I proposed defines a lesion candidate by selecting the most confident voxel as the `peak' and extending the lesion candidate until $40\%$ of its peak confidence. To extract multiple lesion candidates, this process is repeated. See \Cref{fig:dynamic-threshold-pipeline-large} for an example. 

\input{figures/dynamic-threshold-pipeline-large}


To validate the dynamic extraction of lesion candidates, I compared model performance obtained using the dynamic extraction pipeline against a range of static thresholds, as well as a sample-dependent threshold obtained using Otsu's method and a sample-dependent threshold defined as $40\%$ of the sample's peak. Please note that the latter method is different from the dynamic pipeline because it applies a single threshold and extracts all subsequent `islands', instead of the iterative approach of the dynamic extraction, and is termed `dynamic-fast'. Results for my baseline models (at the time of investigating the dynamic lesion candidate extraction), with 5-fold cross-validation and 5 restarts are shown in \Cref{fig:dynamic-threshold-FROC-performance}. Results for my models trained on automatic annotations (which used soft labels at the time), with 5-fold cross-validation and 3 restarts are shown in \Cref{fig:dynamic-threshold-FROC-performance-AVA}. The dynamic lesion candidate extraction either performs on par or outperforms the best static threshold, across all metrics. Most importantly, the dynamic extraction did not require any tuning, while the static pipeline has different optimal thresholds across metrics and models. 


\input{figures/dynamic-threshold-FROC-performance}
\input{figures/dynamic-threshold-FROC-performance-pseudo-labels}



==> chapters/deprecated/0-abstract-v1.tex <==
Accurate risk stratification and detection of potentially aggressive lesions using non-invasive methods such as bi-parametric MRI is instrumental for the management of prostate cancer. 
% Prostate cancer was the most prevalent cancer for men in Europe in 2020. % ecis2021
% Treatment and management options for prostate cancer 
% The majority of men over 60 years of age have some form of PCa, but 
% Only a small portion of prostate cancer is aggressive cancer that will metastasise. 
% When diagnosed before metastasis, prostate cancer can be treated effectively, resulting in %a mortality rate of $23\%$ 
% prostate cancer to be the third leading cause of cancer deaths for men in Europe in 2020. % ecis2021
% Treatment is not risk-free, so accurate diagnosis of aggressive prostate cancer is important. The golden standard to diagnose prostate cancer before treatment is to perform an MRI-targeted biopsy. Because even these biopsies are associated with the risk of complications, % \citep{yang2021morphological}
% it is important to accurately stratify aggressive prostate cancer using non-invasive methods. A bi-parametric MRI scan is the most effective non-invasive method to discriminate between aggressive and indolent prostate cancer. %, % eldred2021population
% with high sensitivity but low specificity. 
% 
% Simulate shorter abstract by skipping last part
% % introduce CAD system
Current deep learning based computer aided diagnosis models are either trained on a limited number of biopsy-confirmed studies, or radiology-based training ground truth, \color{blue}which is less than the training of an experienced radiologist. \color{black}
% There currently exist Machine Learning models for Computer Aided Diagnosis of aggressive prostate cancer, which can help radiologists in their diagnosis. However, these models are not yet able to surpass human expert performance, so further improvements are needed. % Schelb? + voorbeeld in klinkiek?
In this work, we propose a hybrid training framework that uses over \color{red}\numTrainingVisitsBiopsiedFullDataset\ visits with patient-level pathology findings, as well as over \color{black}\numTrainingVisitsFullDataset\ prostate MRI visits in total. 

For two thirds of our training samples, we generate pseudo-labels by amending model predictions using information automatically extracted from radiology or pathology reports.
% For two thirds of our training samples, we generate pseudo-labels by combining model predictions with the number of clinically significant lesions we extract from the radiology or pathology report. % simplify this. also not 'combine' but other wording
These model predictions are from a model trained on the other one third of the training samples, for which the clinically significant prostate cancer lesions were manually delineated. % To extract the number of clinically significant lesions from the reports, we developed a rule-based natural language processing script. 


% To achieve this large training set, we combine natural language processing to extract the PI-RADS or Gleason scores from Radiology or Pathology reports, with model predictions to create pseudo-labels.  

\textit{Results:} 
\color{blue}Extending the training set with pseudo-labels improves the patient-level risk stratification to an AUROC of \perfMPseudoLabelsAll\ (from \perfMManualDelineations, \statMPseudoLabelsAllBetterThanMManualDelineations). 

\vspace{3em}
\color{red}For RSNA: only write about using pseudo-label to incorporate more studies.\color{black}
\color{blue}Note: results are currently based on the validation sets, with scores automatically extracted from the reports. Positive label: GGG$\geq 2$, negative label: $GGG=1$ or $PI-RADS \leq 2$

==> chapters/deprecated/0-abstract-v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
\abstractSection{Purpose:}
% use 'deep learning' to end up in search queries?
To improve risk stratification of clinically significant prostate cancer (csPCa) with a 3D deep learning detection model, by augmenting the largest prostate MRI dataset reported in literature to date. 
%by leveraging the largest, partially annotated, prostate MRI dataset reported in literature to date. %, for training a deep learning detection model. 
% To improve performance of patient-level clinically significant prostate cancer (csPCa) risk stratification with deep learning, %by leveraging over \numTrainingVisitsUnlabelledFullDataset\ automatically segmented, as well as \numTrainingVisitsLabelledFullDataset\ manually segmented prostate exams. 
% by using both \numTrainingVisitsLabelledFullDataset\ manual and \numTrainingVisitsUnlabelledFullDataset\ automatically segmented prostate exams. 
% Current deep learning models for computer aided diagnosis are either trained on a limited number of biopsy-confirmed studies, or radiology-based training ground truth, \color{blue}which is less than the training of an experienced radiologist. \color{black}


%%%%%%%%%%%%%%%%%%%%%%%%%
\abstractSection{Materials and Methods:}
% data
This retrospective study included \numbpMRIVisitsFullDataset\ prostate bpMRI studies (axial T2-weighted, high b-value ($\geq 1400$) and apparent diffusion coefficient scans) from \numbpMRIPatientsFullDataset\ consecutive patients, with elevated PSA or clinical suspicion of PCa, between 2014-2020 for training. All studies were evaluated by experienced radiologists during clinical routine. 
% For this retrospective study, axial T2-weighted, high b-value ($\geq 1400$) and apparent diffusion coefficient scans from consecutive prostate MRI studies with elevated PSA or clinical suspicion of PCa between 2014 and 2020 were used for training.
% For this retrospective study, the axial T2-weighted, high b-value ($\geq 1400$) and apparent diffusion coefficient scans from consecutive prostate MRI exams between 2014 and 2020 were used for training. 
% All \numTrainingSamplesProposedPIRADS\ studies were evaluated by experienced radiologists as part of clinical routine. 
The findings in \numTrainingSamplesManualPIRADS\ studies were manually segmented. 
% As part of clinical routine, the studies were evaluated by experienced radiologists. 
% and received a targeted \color{blue}and/or \color{black} systematic biopsy if they were suspicious for prostate cancer. 
% Lesions with PI-RADS 4 or 5 
% PI-RADS 4 and 5 lesions 
% were manually segmented for 2,659 studies. %between 2016 and 2018. 

% PI-RADS lesions $\geq 4$
% for studies between 2016 and 2018 were manually segmented. % January ~ and August ~?
% Lesions with PI-RADS $\geq 4$ 

% pseudo-labels
% We propose a hybrid framework, \frameworkName, to augment our detection model with more training data. 
We propose a hybrid framework to augment our detection model with more training data. 
% To train a detection model on visits without expert csPCa segmentations, we propose a hybrid framework, \frameworkName. 
After training %a detection model 
with expert csPCa segmentations, we generate automatic cancer segmentations 
% v1: by amending the model predictions using information automatically extracted from the radiology report. 
% v2: by using information automatically extracted from the radiology report to amend the model predictions. 
by masking our model predictions with the number of csPCa lesions automatically extracted from radiology reports. 
An augmented detection model is then trained jointly on manual and automatically generated csPCa segmentations. 
% A student detection model is then trained jointly on manually segmented studies from 2016-2018 and automatically segmented studies from 2014, 2015, 2019 and 2020. 
% A student detection model is then trained jointly on manual segmentations and automatically generated segmentations for the remaining studies. 

% In this work, we propose a hybrid training framework that uses over \numTrainingVisitsFullDataset\ prostate MRI visits in total. 
% For two thirds of our training samples, we generate pseudo-labels by amending model predictions using information automatically extracted from radiology reports.
% These model predictions are from a model trained on the other one third of the training samples, for which the clinically significant prostate cancer lesions were manually segmented. 

% evaluation

Models trained on expert or augmented cancer segmentations
% Expert and augmented models 
are evaluated on \numZGTVisits\ visits of \numZGTVisits\ consecutive men with elevated PSA or clinical suspicion of prostate cancer from an independent, external, centre. 
Ground truth is provided by MR-guided and TRUS-guided biopsies, and radical prostatectomy when available. % csPCa is defined as Gleason grade group $\geq 2$, and studies with $\geq 1$ csPCa lesions are considered positive. %Positive case-level labels are defined as having at least one csPCa lesion. 
Studies are considered positive if they have at least one Gleason grade group $\geq 2$ lesion (csPCa).
% Studies with at least one Gleason grade group $\geq 2$ lesion (csPCa) are considered positive.

% metrics and statistical test
We trained our models on expert and augmented segmentations with 5-fold cross-validation and 5 restarts. 
% We used case-level biopsy-confirmed csPCa AUROC % Area Under the Receiver Operator Curve (AUROC) of predicting positive studies
% Patient-level? 
Diagnostic performance was evaluated using the Area under the Receiver Operating Characteristic curve (AUROC). We performed a permutation test to obtain the statistical significance level. 
% We used case-level Area Under the Receiver Operator Operating Curve (AUROC) of predicting positive studies
% to compare the models and performed a permutation test to obtain the statistical significance level. 

%%%%%%%%%%%%%%%%%%%%%%%%%
\abstractSection{Results:}
% To train the detection model, \numTrainingSamplesProposedPIRADS\ prostate MRI visits were used (\distPSALevelsRUMC). For evaluation of the model, \numZGTVisits\ visits from the first external institution were used (\distPSALevelsZGT) and \numUMCGVisits\ visits from the second external institution (\distPSALevelsUMCG). %to evaluate the model. 
% 
Augmenting the training set with automatic csPCa segmentations guided by report findings, 
% \frameworkName\ 
significantly improves the case-level risk stratification of csPCa. For the external test set, the AUROC increased from \perfTeacherAUCZGT\ to \perfStudentAUCZGT\ (\statStudentBetterThanTeacherZGT). % The AUROC increased from \perfTeacherAUCUMCG\ to \perfStudentAUCUMCG\ (\statStudentBetterThanTeacherUMCG) for the second test set. 

On the external test set, experienced radiologists had a sensitivity of \perfRadiologistSensitivityZGT\ at \perfRadiologistSpecificityZGT\ specificity. 
% radiologist's sensitivity
At the same sensitivity, adding automatic segmentations improved the model's specificity from \perfTeacherSpecificityZGT\ to \perfStudentSpecificityZGT\ (\statStudentBetterThanTeacherZGTSpecificity). 
% Our improved Student model reached the same sensitivity at \perfStudentSpecificityZGT, while the Teacher model had a specificity of \perfTeacherSpecificityZGT.
% For the second test set, the radiologist's sensitivity of \perfRadiologistSensitivityUMCG\ at \perfRadiologistSpecificityUMCG\ specificity is reached by our improved model at a specificity of \perfStudentSpecificityUMCG, while the initial model had a specificity of \perfTeacherSpecificityUMCG. 
% For the second test set, the radiologist's sensitivity was \perfRadiologistSensitivityUMCG\ at \perfRadiologistSpecificityUMCG\ specificity. At the same sensitivity, using \frameworkName\ improved the model's specificity from \perfTeacherSpecificityUMCG\ to \perfStudentSpecificityUMCG. 

% On the first test set, our model achieved a sensitivity of \perfStudentSensitivityZGT\ at a specificity of \perfStudentSpecificityZGT, compared to a sensitivity of \perfRadiologistSensitivityZGT\ at a specificity of \perfRadiologistSpecificityZGT\ for expert radiologists. On the second test set, our model achieved \perfStudentSensitivityUMCG\ sensitivity at  \perfStudentSpecificityUMCG\ specificity, compared to  \perfRadiologistSensitivityUMCG\ sensitivity at \perfRadiologistSpecificityUMCG\ specificity of expert radiologists. 


%%%%%%%%%%%%%%%%%%%%%%%%%
\abstractSection{Conclusion:}
% Augmented 
% Training with manually and automatically segmented prostate cancer in bpMRI using \frameworkName\ 
Augmenting training with automatic report driven segmentations of prostate cancer in bpMRI
% Including weakly labelled prostate MRI visits with \frameworkName\ 
significantly improved the risk-stratification of the deep learning prostate cancer detection model. 


%%%%%%%%%%%%%%%%%%%%%%%%%
\abstractSection{Clinical Relevance:}
Risk stratification for clinically significant prostate cancer using prostate MRI is instrumental to reduce over-treatment. Deep learning can assist, but requires expensive expert segmentations. 
% has potential to assist in and speed up this risk assessment.



% scrap
% overcome manual labeling bottlenecks in the machine learning pipeline.
% Automatically annotating studies 
% Automatically annotating studies based on clinical reports would allow datasets to grow significantly, without additional manual effort. 
% If studies can be annotated based on clinical reports, datasets can grow to all available visits without additional manual effort. 
% We investigate how unlabelled studies paired with reports can be leveraged to improve deep learning detection performance. 


==> chapters/deprecated/0-abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
% \abstractSection{Purpose:}
% use 'deep learning' to end up in search queries?
% To improve risk stratification of clinically significant prostate cancer (csPCa) with a 3D deep learning detection model, by augmenting the largest prostate MRI dataset reported in literature to date. 
%by leveraging the largest, partially annotated, prostate MRI dataset reported in literature to date. %, for training a deep learning detection model. 
% To improve performance of patient-level clinically significant prostate cancer (csPCa) risk stratification with deep learning, %by leveraging over \numTrainingVisitsUnlabelledFullDataset\ automatically segmented, as well as \numTrainingVisitsLabelledFullDataset\ manually segmented prostate exams. 
% by using both \numTrainingVisitsLabelledFullDataset\ manual and \numTrainingVisitsUnlabelledFullDataset\ automatically segmented prostate exams. 
% Current deep learning models for computer aided diagnosis are either trained on a limited number of biopsy-confirmed studies, or radiology-based training ground truth, \color{blue}which is less than the training of an experienced radiologist. \color{black}
% 
%== Simple overview of main contributions in this paper ==%
Prostate MRI interpreted by expert radiologists provides the best non-invasive diagnosis of clinically significant prostate cancer (csPCa), but is a resource that is not readily available. 
% Deep learning currently lacks stand-alone performance to 
Deep learning can assist, but lacks stand-alone performance compared to experts. 
% Deep learning currently lacks stand-alone performance compared to experts, hindering its applicability. 
% Deep learning can assist, but currently lacks stand-alone performance. 
Annotating more cases increases model performance, but is expensive. % Increasing the training dataset size improves performance, but is a time-consuming and requires expensive expert annotations. 
% Current deep learning csPCa detection systems lack the quantity of training samples to reach expert-level performance
% Deep learning performance improves with increasing amounts of data
% Deep learning systems perform better with increasing amounts of data, but current systems for prostate cancer detection in MRI are lacking the numbers to reach expert-level performance. 
Experts evaluate diagnostic images during clinical routine, and write their findings in reports. 
% Diagnostic images are evaluated during clinical routine, and come with reports describing the findings. 
% v2:
% We investigate false-postive reduction by postprocessing 
% \blue{augmenting the training set with} 
We investigate how these studies paired with reports can be leveraged to improve deep learning cancer detection performance. 
% We investigate leveraging these unlabelled cases by automatically generating voxel-level annotations. 
% We propose training the csPCa detection model on weakly supervised
% Our proposed labelling procedure is a weakly supervised
% We investigate the automatic generation of voxel-level annotations by combining model predictions with information from reports. 
% We investigate automatically generating voxel-level annotations by postprocessing model predictions using information from the reports. This model is trained on a manually annotated subset of cases 
% We trained this model on a manually annotated subset of cases 
% v1:
% We investigate automatically generating voxel-level annotations, using a model trained on a manually annotated subset of cases and reducing its false-positives with information from the reports. 
% We developed an automatic labelling procedure\footnote{Code for the automatic extraction of report findings and the automatic annotation procedure will be made publicly available before journal submission. } guided by radiology reports from clinical routine, capable of generating high quality voxel-level annotations. % of clinically significant findings. %. 
Our proposed method is to automatically generate voxel-level annotations, guided by the reports. 
We show that a baseline csPCa detection model paired with false-positive reduction based on the reports can automatically generate annotations of high quality. 
% First, we train a csPCa detection model on a manually annotated subset. Then, we generate lesion candidates for the unlabelled cases. To reduce false-positives, we remove lower confidence lesion candidates until we have the same number of lesion candidates as there are csPCa lesions in the report. 
% Our proposed labelling procedure is to parse the report, count the csPCa lesions, 
% and generate annotation by keeping that number of lesion candidates from the csPCa segmentation model. % (ordered by confidence). 
%== Materials ==%
We included \numbpMRIVisitsFullDataset\ prostate bpMRI studies, % (axial T2, high b-value and ADC scans), 
of which \numTrainingSamplesManualPIRADS\ were manually annotated and \numUnlabelledStudiesFullDataset\ were automatically annotated. % resulting in the largest prostate MRI dataset reported in literature to date.
% All studies were evaluated by experienced radiologists during clinical routine. 
% with elevated PSA or clinical suspicion of PCa, between 2014-2020 for training.
% These automatic annotations enabled us to use \numUnlabelledStudiesFullDataset\ additional prostate MRI visits, on top of \numManualDelineationsFullDataset\ manually annotated visits, resulting in the largest prostate MRI dataset reported in literature to date. %, without the large manual annotation time investment for. 
% which enabled , without the . 
% We evaluated the automatic annotation procedure using the manual annotations, and found that our score extraction correctly identified \nsig\ 
% % We evaluated the quality of the automatic annotations against the manual annotations, and observed that our score extraction correctly identified \nsig\ % the number of clinically significant report findings 
% for \perfAutomaticFindingExtractionAccuracy\ of the visits, 
% our prostate cancer segmentation model correctly localised \perfLesionLocalisationnnUNetSensitivityFiltered\ of the lesions, 
% and the automatic annotations of correctly localised lesions have good spatial congruence with Dice similarity coefficients of \perfLesionSegmentationAVAnnUNetMatched. 
We evaluated the automatic annotation quality on the manually annotated subset: 
our score extraction correctly identified the number of csPCa lesions for \perfAutomaticFindingExtractionAccuracy\ of the reports and
our csPCa segmentation model correctly localised \perfLesionLocalisationnnUNetSensitivityFiltered\ of the lesions. 
% and the automatic annotations of correctly localised lesions have good spatial congruence, with Dice similarity coefficients of \perfLesionSegmentationAVAnnUNetMatched. 
We evaluated prostate cancer detection performance on \numZGTVisits\ visits from an external centre with histopathological ground truth. % provided by MR-guided and TRUS-guided biopsies, or radical prostatectomy when available.
Augmenting the training set with 
% Including 
automatically labelled visits improved patient-based diagnostic area under the receiver operating characteristic curve from \perfZGTAUCnnUNetManual\ to \perfZGTAUCnnUNetManualAndAutomatic\ (\statZGTAUCnnUNetManualBetterThanManualAndAutomatic) and improved lesion-based diagnostic partial area under the free-response operating characteristic curve ($0.01-2.5$ false positives per case) from \perfZGTpAUCnnUNetManual\ to \perfZGTpAUCnnUNetManualAndAutomatic\ (\statZGTpAUCnnUNetManualBetterThanManualAndAutomatic), with $mean \pm std.$ over 15 independent runs. 
% significantly improved prostate cancer detection performance, as evaluated on \numZGTVisits\ visits from an independent, external, centre with ground truth provided by MR-guided and TRUS-guided biopsies, or radical prostatectomy when available. 
% Studies are considered positive if they have at least one Gleason grade group $\geq 2$ lesion. 
% Patient-based diagnostic AUROC increased from \perfZGTAUCnnUNetManual\ to \perfZGTAUCnnUNetManualAndAutomatic\ (\statZGTAUCnnUNetManualBetterThanManualAndAutomatic) and lesion-based diagnostic pAUC increased from \perfZGTpAUCnnUNetManual\ to \perfZGTpAUCnnUNetManualAndAutomatic\ (\statZGTpAUCnnUNetManualBetterThanManualAndAutomatic), with $mean \pm std.$ over 15 independent runs. 
Code available at github.com/\blue{pending}. 
% \blue{Code for the automatic extraction of report findings and the automatic annotation procedure will be made publicly available before journal submission. }
% Patient-based diagnostic area under the receiver operating curve (AUROC)

% Prostate cancer detection models trained on manual or manual+automatic annotations are evaluated on \numZGTVisits\ visits of \numZGTVisits\ consecutive men with elevated PSA or clinical suspicion of prostate cancer from an independent, external, centre. Ground truth for these visits is provided by MR-guided and TRUS-guided biopsies, or radical prostatectomy when available. Studies are considered positive if they have at least one Gleason grade group $\geq 2$ lesion (csPCa).
% Augmenting the training dataset with automatically labelled visits improved patient-based AUROC from \perfTeacherAUCZGT\ to \perfStudentAUCZGT\ (\statStudentBetterThanTeacherZGT) and lesion-based pAUC from \perfTeacherpAUCZGT\ to \perfStudentpAUCZGT\ (\statStudentBetterThanTeacherFROCZGT) over 25 runs each.
% 
% 
% 

% Deep learning systems perform better with increasing amounts of data, but current systems for prostate cancer detection in MRI are lacking the numbers to reach expert-level performance. 
% We developed an automatic labelling procedure guided by radiology reports from clinical routine, capable of generating high quality voxel-level annotations. 
% First, we parse the radiology report to extract the number of clinically significant findings (nsig), 
% and then generate annotation by keeping the nsig most confident lesion candidates from a prostate cancer segmentation model. 
% We included A prostate bpMRI studies (axial T2, high b-value and ADC scans), 
% of which C were manually annotated and B were automatically annotated, 
% resulting in the largest prostate MRI dataset reported in literature. We evaluated the quality of the automatic annotations against the manual annotations, and observed that our score extraction correctly identified nsig for D of the visits, 
% our prostate cancer segmentation model correctly localised X of the lesions, 
% and the automatic annotations of correctly localised lesions have good spatial congruence with Dice similarity coefficients of Y. 
% Augmenting the training set with automatically labelled visits improved prostate cancer detection performance, as evaluated on Z visits from an external centre with ground truth provided by MR-guided and TRUS-guided biopsies, or radical prostatectomy when available. Studies are considered positive if they have at least one Gleason grade group Q lesion. Patient-based AUROC increased from R to S (T) and lesion-based pAUC increased from A to S (D), with mean ± std. over 25 independent runs. 

==> chapters/deprecated/1-introduction-scrap-paper.tex <==

%%%%%%%%%%%%%%%%%
% PCa detection %
%%%%%%%%%%%%%%%%%

% schelb2019classification: 
% U-Net with sextant calibration of predictions
% Trained on biopsy-confirmed delineated lesions
% Used prostate segmentation as specific 'benign' class, rather than full MRI scan

% sanford2020deep:
% Classification of MRI in PI-RADS 2, 3, 4 or 5

% arif2020clinically:
% U-Net trained on biopsy-confirmed delineated lesions
% Uses (also?) low-risk patients to train and evaluate model
% Weak: Excludes visits with (P<=2 and GGG>=2) or (MRGB GGG <= 1 and TRUS GGG >= 2) from training and evaluation
% Strong: Divides performance in lesion volume >0.03cc, >0.1cc and >0.5 

% yu2020deep:
% Trained on PI-RADS ≥ 3, 3D bounding boxes in MRI by an "expert radiologist with 4 years of experience" (= four years of experience in radiology and subspecialty training in prostate MRI examinations)
% (evaluated on ProstateX, which uses PI-RADS as ground truth)

% yu2020false
% 2170 samples, 1736 for training, PI-RADS only. Classification network for False Positive reduction. 

% sanyal2020automated: 77 biopsy patients divided over train (57), val (20), test (20), single circumcision on slice with largest csPCa section

% aldoj2020semi: 

% bhattacharya2020corrsignet (also with Seetharaman)

% cao2021performance:
% FocalNet evaluation versus GU 

% seetharaman2021automated (Stanford) <-- also uses automatically generated labels! Automatically segments PCa on histopathology, and registers pathology slice onto MRI to obtain labels. Could we do the same thing but with orders of magnitude more slices/scans?

% saha2021end

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pseudo-labels in general %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Recent ImageNet leaderbord holders:
% - CoAtNet: Marrying Convolution and Attention for All Data Sizes (https://paperswithcode.com/paper/coatnet-marrying-convolution-and-attention)
% - Scaling Vision Transformers (https://paperswithcode.com/paper/scaling-vision-transformers)
% - Meta Pseudo Labels (https://paperswithcode.com/paper/meta-pseudo-labels)
% - EfficientNet-L2-475 (SAM) (https://paperswithcode.com/paper/sharpness-aware-minimization-for-efficiently-1)
% - ViT-H/14 (https://paperswithcode.com/paper/an-image-is-worth-16x16-words-transformers-1)
% - FixEfficientNet-L2 (https://paperswithcode.com/paper/fixing-the-train-test-resolution-discrepancy-2)
% - BiT-L (ResNet) (https://paperswithcode.com/paper/large-scale-learning-of-general-visual)
% - NoisyStudent (EfficientNet-B7) (https://paperswithcode.com/paper/self-training-with-noisy-student-improves)
% - FixResNeXt-101 32x48d (https://paperswithcode.com/paper/fixing-the-train-test-resolution-discrepancy)

% > 3yrs ago:
% - ResNeXt-101 32x48d ("Exploring the Limits of Weakly Supervised Pretraining", 2 May 2018) (https://paperswithcode.com/paper/exploring-the-limits-of-weakly-supervised)
% (before that, AmoebaNet-A, which is the last NOT to use extra training data)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pseudo-labels in medical imaging %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Bulten2020, Automated Gleason Grading of Prostate Biopsies using Deep Learning
% Gündel2021, Robust classification from noisy labels- Integrating additional knowledge for chest radiography abnormality assessment

% Notes from Lesie: 
% aden == gland
% tumor in epithelium == carcinoma
% all tumors we call "prostate cancer" are tumors in epithelium, i.e. carcinoma. Other tumors could be metastatis from other regions, but are much more rare and not called "prostate cancer"
% epithelium is the thing that bounds something, for example the glands inside a prostate (not sure if this is worded properly)



% Bulten2020: "With 1.2 million new prostate cancer cases each year1, a high incidence-to-mortality ratio, and risk of overdiagnosis and overtreatment2,3, there is a strong need for accurate assessment of patient prognosis."

\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduce prostate cancer and the importance of MRI in the management of csPCa %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Prostate cancer (PCa) has 1.2 million new cases each year \citep{GCS2020}, a high incidence-to-mortality ratio and risks associated with treatment and biopsy; making non-invasive diagnosis of clinically significant prostate cancer (csPCa) crucial to reduce both overtreatment and unnecessary (confirmatory) biopsies \citep{stavrinides2019mri}. Multiparametric MRI (mpMRI) scans interpreted by expert prostate radiologists % ($> 20$ years of experience) 
provide the best non-invasive diagnosis \citep{eldred2021population}, but is a limited resource that can't be leveraged freely. %but is a resource that is not readily available. %
% expert: ($> 20$ years of experience) 
% long version:
%Due to its high incidence-to-mortality ratio and risk associated with treatment \citep{stavrinides2019mri}%\blue{\citep{schroder2012prostate, cooperberg2010time}}
%, accurate diagnosis of clinically significant prostate cancer (csPCa) is crucial. 
%
%
% Prostate cancer (PCa) had the highest incidence rate among all cancers for men in Europe in 2020 \citep{ecis2021}. % ecis2021
% Only a portion of PCa is aggressive cancer that will metastasise, and when diagnosed before metastasis, prostate cancer can be treated effectively. These two factors combined result in prostate cancer to cause the third most cancer deaths for men in Europe in 2020 \citep{ecis2021}. 
% Prostate cancer (PCa) was the most prevalent cancer for men in Europe in 2020 \citep{ecis2021}. % ecis2021
% Only a small portion of PCa is aggressive cancer that will metastasise (csPCa). 
% When diagnosed before metastasis, prostate cancer can be treated effectively, resulting in a mortality rate of $23\%$ and third leading cause of cancer deaths for men in Europe in 2020 \citep{ecis2021}. 
% Treatment is not risk-free, so accurate diagnosis of clinically significant prostate cancer (csPCa) is crucial. 
%  golden standard to diagnose 
% The most reliable way to diagnose prostate cancer without extracting the prostate 
% The most powerful prognostic marker for prostate cancer prior to treatment 
% is to perform an MRI-targeted and TRUS biopsy \citep{eldred2021population, radtke2016multiparametric}. The MRI-targeted biopsy cores are taken at the locations that are found to be suspicious on the MRI scan, so high sensitivity of csPCa lesions on MRI is important for an accurate prognosis. Unfortunately, performing biopsies is associated with the risk of complications, and for low-risk patients (confirmatory) biopsies introduce more risk than the prognosis will resolve \citep{stavrinides2019mri}. To reduce the number of unnecessary biopsies, accurate and non-invasive risk stratification of aggressive prostate cancer is required, for which multi-parametric MRI (mpMRI) scans have shown to be most effective %.  % Multi-parametric MRI (mpMRI) scans have shown to be 
% For the decision whether to perform a biopsy, it is important to accurately stratify aggressive prostate cancer using non-invasive methods on a patient-level. 
% A multi-parametric MRI scan (mpMRI) is the most effective non-invasive method to discriminate between csPCa and non-aggressive lesions in the prostate %, with high sensitivity but low specificity 
% \citep{eldred2021population, stavrinides2019mri}. MRI scans and their interpretation are thus instrumental both for patient-level risk stratification and lesion identification. \\
% Therefore, to manage prostate cancer, both patient-level risk stratification and lesion identification on MRI are instrumental. the MRI serves both the purpose of determining the loca
%
% this work aims to improve both patient-level risk stratification to aid the decision whether to perform a biopsy, and the localisation of aggressive prostate cancer to aid the decision where to perform a biopsy. %focuses both on obtaining the best patient-level diagnosis to aid the decision whether to perform a biopsy, and on localisation of the lesions to aid the decision where to perform a biopsy. 
% \blue{The driving machine learning models are 3D detection models that can give voxel-level predictions. We use the same model architectures as used in prior work \citep{saha2021end}, which are based on 3D UNets and detailed in \Cref{sec:methods}. The goal of this work is to push the performance of these models by utilising the largest prostate cancer dataset reported in literature to this date. }
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduce CAD for the interpretation of MRI %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Computer-aided diagnosis (CAD) can assist radiologists to diagnose csPCa, but lacks stand-alone performance compared to expert radiologists \citep{schelb2019classification, cao2021performance, saha2021end, seetharaman2021automated}. % expert prostate radiologists

% Related fields where CAD is better than radiologists:
% - Lung cancer (Data: NLST; 29,541 training cases from 10,306 patients, 398 of whom developed biopsy-confirmed cancer within 1 year of a LDCT. Ardila2019)
% - Melanoma (Data: 16,114 training cases from 12,399 patients; Coz2020, "A deep learning system for differential diagnosis of skin diseases")
% - Breast cancer (Data: approx. (not entirely clear) 121,850 patients; McKinney2019, "International evaluation of an AI system for breast cancer screening")
CAD systems in fields where clinical experts are matched or outperformed typically use very large training datasets. Top performing deep learning systems used 29,541 training cases (10,306 patients) for the detection of lung cancer \citep{ardila2019end}, 121,850 training cases (121,850 women) for the detection of breast cancer \citep{mckinney2020international} and 16,114 training cases (12,399 patients) for the classification of skin diseases \citep{liu2020deep}. %These training datasets are significantly larger than the datasets used for prostate cancer detection. 

Datasets used for prostate cancer detection and diagnosis are significantly smaller. 
% Other works often use histopathology based ground truth to train their models, 
% Clinically significant prostate cancer (csPCa) detection is an active research topic, and many Machine Learning models for Computer Aided Diagnosis (CAD) of csPCa have been developed %
% introduce CAD system
% In related work, multiple Machine Learning models for Computer Aided Diagnosis (CAD) of csPCa have been developed 
% There currently exist multiple Machine Learning models for Computer Aided Diagnosis (CAD) of csPCa %, which can help radiologists in their diagnosis \
% \citep{schelb2019classification, sanford2020deep, arif2020clinically, yu2020deep, yu2020false, sanyal2020automated, aldoj2020semi, bhattacharya2020corrsignet, cao2021performance, seetharaman2021automated, saha2021end}. 
Studies tackling prostate cancer detection in MRI by training on histopathological annotations, use datasets with \numTrainingSamplesBhattacharya -\numTrainingSamplesNetzerBiop\ (median: \numTrainingSamplesBiopMedian) samples to train their deep learning system \citep{schelb2019classification, arif2020clinically, sanyal2020automated, aldoj2020semi, bhattacharya2020corrsignet, cao2019joint, seetharaman2021automated, netzer2021fully}. 
Approaches using radiologically-estimated annotations used \numTrainingSamplesSanford -\numTrainingSamplesSaha\ (median: \numTrainingSamplesRadiolMedian) training samples \citep{sanford2020deep, yu2020deep, yu2020false, saha2021end}. 

Between these two types of annotations there are important trade-offs. Histopathological annotations provide high quality ground-truth annotations \citep{radtke2016multiparametric}, but also inherently considers intermediate to high risk patients, has risk associated with acquisition \citep{loeb2011complications} and is expensive \citep{altok2018cost}. Alternatively, the less accurate radiologically-estimated ground truth (reported using Prostate Imaging Reporting and Data System: Version 2 (PI-RADS)) can be used. These annotations allow the inclusion of all patients who received an MRI examination and covers the complete distribution of patients encountered in clinical practice. It is unclear how the benefits of a wider training cohort and larger training size compare against the downside of more noise in the training annotations. 

% For patients suspected of prostate cancer who received a biopsy or prostatectomy after the MRI visit, the histological finding can be retrospectively mapped to the MRI scan. 
% Including patients with a biopsy or prostatectomy after the prostate MRI visit allows to retrospectively annotate the histopathological finding in the MRI scan. 
% This approach provides high quality ground-truth annotations, but also inherently considers intermediate to high risk patients exclusively and is very expensive to obtain. 
% Most prostate cancer detection studies included patients with an MRI visit before a biopsy or radical prostatectomy, and retrospectively annotated the histopathological finding in the MRI scan \citep{schelb2019classification, arif2020clinically, sanyal2020automated, aldoj2020semi, bhattacharya2020corrsignet, cao2021performance, seetharaman2021automated}. 
% The histopathological ground truth used in these studies varied from whole-mount histopathology (WMHP), to both MR and TRUS guided biopsies, or unspecified. % The histopathological ground truth used in these studies varies, \citep{bhattacharya2020corrsignet} and \citep{cao2021performance} use whole-mount histopathology (WMHP) exclusively, \citep{seetharaman2021automated} uses WMHP or biopsy, \citep{schelb2019classification} and \citep{arif2020clinically} uses both MR and TRUS guided biopsies and \citep{sanyal2020automated} and \citep{aldoj2020semi} don't specify how their histopathological ground truth was derived. 
% The training ground truths used in these studies are very accurate, WMHP is considered to be the golden standard, and the combination of MR and TRUS guided biopsies is estimated to have a sensitivity of $97\%$ \citep{radtke2016multiparametric}. The limitation of these ground truths is the high cost associated with obtaining them, and the inherent selection of intermediate or high risk patients. 
% The training ground truths used in these studies are very accurate, but also expensive to obtain and inherently select intermediate or high risk patients. 
% Due to the expensive ground truth and selection of intermediate/high risk patients, these studies include only a limited number of training cases
% As a result, studies opting for this training ground truth used only 
% \numTrainingSamplesSchelb\ \citep{schelb2019classification}, \numTrainingSamplesArif\ \citep{arif2020clinically}, \numTrainingSamplesSanyal\ \citep{sanyal2020automated}, \numTrainingSamplesAldroj\ \citep{aldoj2020semi}, \numTrainingSamplesBhattacharya\ \citep{bhattacharya2020corrsignet}, \numTrainingSamplesCao\ \citep{cao2019joint}, \numTrainingSamplesSeetharaman\ \citep{seetharaman2021automated} and \numTrainingSamplesNetzerBiop\ \citep{netzer2021fully}
% \numTrainingSamplesBhattacharya -\numTrainingSamplesNetzerBiop\ (median: \numTrainingSamplesBiopMedian) samples to train their deep learning system \citep{schelb2019classification, arif2020clinically, sanyal2020automated, aldoj2020semi, bhattacharya2020corrsignet, cao2019joint, seetharaman2021automated, netzer2021fully}. % training samples, respectively. 
% Alternatively, radiologically-estimated ground truth (reported using Prostate Imaging Reporting and Data System: Version 2 (PI-RADS)) can be used, allowing the inclusion of all patients who received an MRI examination. 
% While these radiologically-estimated ground truths are less accurate, 
% they are readily available and encompass the complete distribution of patients encountered in the clinical workflow. 
% they are also more readily available, which is clearly reflected in the number of training samples used by these approaches.
% Approaches using radiologically-estimated ground truths used \numTrainingSamplesSanford -\numTrainingSamplesSaha\ (median: \numTrainingSamplesRadiolMedian) training samples \citep{sanford2020deep, yu2020deep, yu2020false, saha2021end}. 
% \newcommand\numTrainingSamplesYuDetection{1,502} % unclear about train/val split, this includes everything
% \newcommand\numTrainingSamplesYuFPReduction{1,736} % did not use cross-validation, this is the 80% for training
% \newcommand\numTrainingSamplesSaha{1,950} % from 1879 patients
% Clinical practice for radiologically-estimated ground truth is to follow the Prostate Imaging Reporting and Data System (PI-RADS): Version 2 \citep{weinreb2016pi}. 

% \citep{sanford2020deep, yu2020deep, yu2020false, saha2021end}
% The other studies use the radiologists' PI-RADS scores to train their models. While these ground truths are less accurate, they are also more readily available, which is clearly reflected in the number of training samples used by these approaches. The PI-RADS based approaches used up to \numTrainingSamplesSaha\ samples, compared to the maximum of \numTrainingSamplesCao\ training samples for histopathology based ground truth. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduce need for many labelled training samples %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These works share an important limitation. 
% We believe these works share an important limitation for their applicability to the clinical workflow. 
% 
% Radiologists are trained on at least 1000 MRI visits before being \textit{expert} \citep{de2020esur}. Expecting a deep learning algorithm to perform similar to expert radiologists when trained on fewer samples ($\leq$ \numTrainingSamplesNetzerBiop) is therefore unrealistic. %
% 
% All prostate cancer detection methods are either trained on a limited number of MRI visits ($\leq 804$), or use radiology-estimated ground truth exclusively. During the training of a radiologist, he or she is typically trained on at least 1000 MRI visits before being considered `experienced'. It is therefore unrealistic to expect a Machine Learning algorithm %, which are considered data-hungry, 
% to perform similar to expert radiologists when trained on fewer samples. 
% The issue with training on radiology-estimated ground truth is the relatively high error rate of the annotations, compared to biopsy based ground truth. 

Prior work investigated the effect of training set size on prostate cancer detection performance, with radiologically-estimated ground truth for training and testing \citep{hosseinzadeh21deep}. This work 
% \blue{Prior work investigated the effect of training a prostate cancer detection model with radiologically-estimated labels, while evaluating performance on a test set with accurate histopathological labels. }
% Prior work trained a prostate cancer detection model with radiologically-estimated labels, while evaluating performance on a test set with accurate histopathological labels \citep{saha2021end, hosseinzadeh21deep}. 
% These works show that prostate cancer detection models can be trained effectively using radiologically-estimated annotations. 
% Prior work shows deep learning csPCa detection models can generalise from noisy radiologically-estimated training labels to histopathological testing labels \citep{saha2021end, hosseinzadeh21deep}. %, but lacks stand-alone performance compared to expert radiologists.
% \citep{hosseinzadeh21deep} 
shows patient-based area under the receiver operating characteristic curve (AUROC) for their internal test set increased logarithmically between \numTrainingCasesHosseinzadehStart\ and \numTrainingCasesHosseinzadehEnd\ training cases, from an AUROC of \RUMCAUCHosseinzadehStart\ to \RUMCAUCHosseinzadehEnd. If this trend continues, it requires tens of thousands of annotated cases to reach expert performance, which is in concordance with related fields. 
% it requires about 7,500 training cases to reach an AUROC of $90\%$ and about 20,000 training cases to reach an AUROC of $92\%$. 
% Another aspect to consider is that $6–25\%$ of clinically significant prostate cancers are not visible on mpMRI \citep{barentsz2016synopsis}, so neither histopathological nor radiologically-estimated training annotations are without noise. 

% The number of training samples is significantly higher for approaches using radiologically estimated ground truth, but these have many false positive annotations compared to the histopathological ground truth. 
% Radiologically estimated ground truths have many false positives, compared to a biopsy based ground truth. 
% While radiologists attend regular meetings with pathologists to discuss the lesions that were discordant with the radiological estimation, this feedback is not incorporated when training a model. % on PI-RADS ground truth. 
% Radiologists attend regular meetings to discuss which lesions turned out to be non-cancerous, and thus receive accurate feedback. However, this feedback is not incorporated when training a model on PI-RADS ground truth. 
% hosseinzadeh21deep: Deep Learning assisted Prostate CancerDetection on Bi-parametric MRI: Minimumtraining data size requirements and effect ofprior knowledge, should arrive Dec 1 2021
% Prior work shows that a model can generalise beyond noisy radiologically-estimated training labels \citep{saha2021end}, but we hypothesise that it requires a significantly higher number of samples to reach expert level performance. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Automatic labelling - general %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Manually labelling training samples is a time consuming and expensive process. Trained students supervised by experienced prostate radiologists annotated the PI-RADS $\geq 4$ findings in more than three thousand of our institutional prostate MRI studies. According to our main annotator, she requires about eight minutes to annotate a single prostate cancer lesion in 3D. Difficult cases are discussed with radiologists, further increasing the overall time investment. %This means that annotating an additional 4,500 or 17,000 cases would require about 375 or 1,417 working hours, respectively. 
Annotating tens of thousands of cases therefore would incur huge costs and an incredibly large time investment. 

% Large datasets of unlabelled samples can often be acquired at relatively low cost, but require additional steps to be leveraged. %incentivising development of methods to leverage those. 
% Annotation time and cost is a limiting factor in many deep learning fields, making techniques that improve performance using unlabelled samples essential. 
Annotation time and cost is a limiting factor in many deep learning fields, making techniques that leverage unlabelled samples essential to improve performance. % without annotations of the target task
% which has resulted in many approaches to leverage unlabelled samples. 
%which has resulted in the exploration of
% making methods to leverage unlabelled samples invaluable. 
% while large datasets of unlabelled samples can often be acquired at relatively low cost. 
In the natural image domain, leveraging samples without target task annotations %enriching the training dataset with automatically labelled samples 
has proven to be effective, even when manually labelled samples are abundant. 
% Collecting training samples and manual annotations is a time consuming and expensive process. %, especially in the medical domain where trained experts provide the ground truth. 
% In the natural image domain the use of automatically generated labels proved to be very effective, even when manual labels are abundant. 
% In the domain of natural images the use of weakly labelled training samples has been around for several years, and shows improvement even when samples are abundant. 
On ImageNet, with 1.3 million manually labelled training samples, all eight leaderboard holders of the past three years used additional training samples with automatically generated labels. 
% Although the methods to leverage these additional samples varies, all methods use automatic labelling techniques. 
Several approaches were employed, \citep{mahajan2018exploring} used 3.5 billion images from Instagram to pre-train their models by predicting the corresponding hashtag (\textit{transfer learning}); \citep{xie2020self} used a \textit{teacher} model to predict 300 million images scraped from the web and selected 130 million samples to train a new \textit{student} model (\textit{self-training}); %This procedure is repeated several times, where the \textit{Student} model becomes the \textit{Teacher} in the next iteration. 
and in \citep{pham2020meta} the teacher-student approach was pushed further by continuously updating the teacher model with reinforcement learning. 
The other five leaderboard holders focused on different research, but did incorporate automatic labelling techniques to reach state-of-the-art performance.
% did not introduce a novel method for automatically labelling samples, and used one of the aforementioned approaches to reach state-of-the-art performance. \\ 
% In fact, all eight of the ImageNet leaderboard holders over the past three years have used automatic labelling of additional training samples. % Three out of these eight leaderboard holder specifically targeted improving the automatic labelling techinique(?)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Automatic labelling - medical imaging - general approaches %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the medical domain, popular techniques to leverage unlabelled samples include transfer learning from a distant or related task, and self-training with automatically generated labels \citep{cheplygina2019not}. 
Other techniques to leverage unlabelled samples include contrastive learning \citep{chaitanya2020contrastive, sowrirajan2021moco, azizi2021big} and self-supervised representation learning \citep{zhou2019models}. These techniques either pre-train without labels, or use model prediction as true label. 

% In the medical domain, similar techniques are employed to leverage unlabelled samples. 
% In the medical domain, the lack of labelled data is a common problem, even when unlabelled cases are more abundant \citep{cheplygina2019not}. 
% Manually labelling training samples is a time consuming and expensive process, a single prostate cancer lesion takes about \blue{5}\ minutes to annotate in 3D. 
% Automatically labelling training samples has huge potential in the medical imaging domain, because it can produce large datasets that would have been impossible or very expensive to label manually. 
% because it allows for large training datasets without requiring human interaction. %, but is often limited by the available clinical data.  and requires specialised solutions. 
% Automatically labelling training samples in the medical imaging domain is difficult, but has huge potential. 
% automatically labelled training samples are hard to obtain, but have huge potential. % if successfully acquired. 
% Automatically labelled training samples are very important in medical imaging as well, where manual labels often require domain experts, making them very expensive to obtain. 
Some approaches go beyond annotating samples using model predictions only. 
% The technique to generate labels depends both on the target task and available clinical data, and requires a specialised solution. 
% The technique to obtain automatically label training samples is dependent on the target task as well as the available clinical data. 
% v2:
In \citep{bulten2019epithelium} they generated pixel-level epithelium cell annotations for hematoxylin and eosin (H\&E) stained prostate biopsies. After scanning the H\&E stained biopsy, they washed out the slice and treated it with an immunohistochemistry stain. This immunohistochemistry stain highlights the epithelium cells, facilitating precise automatic segmentation. These segmentation masks were subsequently translated to the H\&E stained biopsy, by co-registering the scans. These steps allowed large scale generation of epithelium annotation in H\&E stained biopsies, which would have been impossible to obtain manually. 

% v1:
% For example, in \citep{bulten2019epithelium} their goal is to segment epithelium cells in prostate biopsy slices with the standard hematoxylin and eosin (H\&E) stain. To generate training labels they first scan the H\&E stained biopsy slice, and then wash out the slice and treat it with an immunohistochemistry stain. The epithelium cells are highlighted by this immunohistochemistry stain, which enables their automatic segmentation. The epithelium segmentation masks are then translated to the reference frame of the original H\&E stained biopsy slice by co-registering the scans of the biopsy slice in the two different stains. After these steps they generated a large number of precise epithelium masks for H\&E stained biopsies, which would have been impossible to obtain manually. 
% 
% In this second staining, the cells of interest (epithelium) are easily distinguishable from other cells, and ground truth masks of epithelium cells can be created with relatively little effort. 
% Subsequently, they register the biopsy slice with immunohistochemistry stain to the standard H\&E stain, which can be done very precisely since the biopsy slices are physically the same and only differ in colouring. After these steps they have obtained very accurate pixel-level labels for epithelium cells, without the need for manual segmentation. \\

% v2: 
In \citep{bulten2019automated} they generated pixel-level Gleason score annotations in H\&E stained prostate biopsies. First, they generated precise cancer masks. Then, they extracted the Gleason scores from the pathology reports to classify the cancer masks into Gleason grades. These steps allowed the generation of Gleason score annotations in thousands of prostate biopsies, which would have been infeasible to obtain manually. 

% v1:
% In a later study they push the automatic labelling of biopsy slices to Gleason grade groups \citep{bulten2019automated}. Prostate cancer can only occur in epithelium cells, so they combined a rough cancer detection model with their precise epithelium segmentation model to generate precise prostate cancer masks. 
% % By masking the rough cancer masks with pixel-level epithelium masks, they obtain precise masks of cells with prostate cancer. 
% Subsequently, they used pathology reports to automatically classify the prostate cancer masks into Gleason grade groups, creating pixel-level annotations of all Gleason grade groups. 
% Using this method they were able to automatically annotate prostate cancer cells on 4712 biopsy slices, which would have been infeasible to do by hand. 


% Ilse:
% Tijdens het werk heb ik allerlei schermen open staan, waardoor ik snel kan schakelen. Inmiddels gaan dingen ook gewoon vlot door het veel routinematig handelen. 
% 1. Navigeren naar en openen van de scans, en het rapport er bij pakken: Zeg een minuut, misschien een keer iets meer voor openen van de scans en zoeken van rapport
% 2. Het rapport lezen en de laesies lokaliseren in de scan: Dat verschilt enorm. Wanneer rapport en ProCAD niet overeenkomen dan komt er al denkwerk aan te pas. Wanneer geen puntannotatie is gegeven, of er tussen de annotatie en rapport tegenstrijdige informatie is etc dan moet ik er echt zelf over gaan oordelen  en dan kan het zijn dat ik er zo'n 10/15 minuutjes over doe.
% 3. Het vervolgens intekenen van de laesies: als de lesie is gevonden dan gaat dit vlug, zeg een minuut voor de kleine lesies, en misschien 3 minuut per lesies voor de grotere en onduidelijkere.
% ===> approx. 1 + 5 + 2 = 8 min for positive case. For negative case approx. 1 min? Gives 70% * 1 + 30% * 8 = approx. 3 min / case. 
% Consulting experts for difficult cases significantly increases the time, so ~5 min / case on average?

%%%%%%%%%%%%%%%%%%%%%%%
% % Our contributions %
%%%%%%%%%%%%%%%%%%%%%%%
% In this work we introduce an automatic labelling procedure for prostate cancer detection in MRI. 
In this work, we investigate automatically annotating clinically significant prostate cancer in MRI. 
Similar to \citep{bulten2019automated}, we generate annotations for unlabelled samples using model predictions, guided by information from the reports. 
% Similar to \citep{bulten2019automated}, we guide the model predictions for unlabelled samples using information extracted from reports. 
% 
% Specifically, we use a model trained on manually annotated samples, and steer the model predictions for unlabelled using radiology reports   %, to improve subsequent detection performance. 
% In this work we introduce a framework for automatic segmentation of report findings, \frameworkName, and apply it to prostate cancer detection in bpMRI. 
% v1:
% First, we automatically determine the number of clinically significant findings in the radiology report (PI-RADS $\geq 4$ lesions). Secondly, we train a prostate cancer detection model on a manually labelled subset of our dataset, and create lesion candidates for the unlabelled visits in our dataset. Thirdly, we keep the same number of lesion candidates as significant report findings. 
% v2:
First, we train a prostate cancer detection model on manually annotated visits, 
and generate lesion candidates for the unlabelled visits. Then, we count the number of clinically significant findings (PI-RADS $\geq 4$ lesions) described in the radiology report. %, using a rule-based natural language processing script. % Using the lesion candidates we create voxel-level annotations by keeping the most confident lesion candidates. % We keep the same number of lesion candidates as we found in the report, which results 
Subsequently, we match the lesion candidates to the PI-RADS scores from the report, by matching the most confident lesion candidates to the highest scores. Lesion candidates matched to a PI-RADS $\geq 4$ lesion are saved as csPCa annotation. 
% Subsequently, we keep the same number of lesion candidates as found in the report, 
% Subsequently, we create voxel-level annotations by keeping the \nsig\ most confident lesion candidates, and discard the rest. 
% v3:

% First, we automatically determine the number of clinically significant findings (PI-RADS $\geq 4$ lesions) described in the radiology report. 
% Then, we localise the clinically significant findings using a prostate cancer segmentation model, and store voxel-level annotations for the \nsig\ most confident lesion candidates. 

Our automatic labelling procedure enables us to leverage 
% Using our framework, we are able to leverage 
the largest dataset of MRI scans for prostate cancer detection reported in literature to date. 
We demonstrate the efficacy of our automatically generated annotations by training a prostate cancer detection model jointly on manual and automatic annotations, which significantly outperforms training on manual annotations exclusively. 

==> chapters/deprecated/1-introduction.tex <==
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduce prostate cancer and the importance of MRI in the management of csPCa %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Prostate cancer (PCa) has 1.2 million new cases each year \citep{GCS2020}, a high incidence-to-mortality ratio and risks associated with treatment and biopsy; making non-invasive diagnosis of clinically significant prostate cancer (csPCa) crucial to reduce both overtreatment and unnecessary (confirmatory) biopsies \citep{stavrinides2019mri}. Multiparametric MRI (mpMRI) scans interpreted by expert prostate radiologists % ($> 20$ years of experience) 
provide the best non-invasive diagnosis \citep{eldred2021population}, but is a limited resource that can't be leveraged freely. %but is a resource that is not readily available. %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduce CAD for the interpretation of MRI %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Computer-aided diagnosis (CAD) can assist radiologists to diagnose csPCa, but lacks stand-alone performance compared to expert radiologists \citep{schelb2019classification, cao2021performance, saha2021end, seetharaman2021automated}. 

CAD systems in fields where clinical experts are matched or outperformed typically use very large training datasets. Top performing deep learning systems used 29,541 training cases (10,306 patients) for the detection of lung cancer \citep{ardila2019end}, 121,850 training cases (121,850 women) for the detection of breast cancer \citep{mckinney2020international} and 16,114 training cases (12,399 patients) for the classification of skin diseases \citep{liu2020deep}. 

Datasets used for prostate cancer detection and diagnosis are significantly smaller. 
Studies tackling prostate cancer detection in MRI by training on histopathological annotations, use datasets with \numTrainingSamplesBhattacharya -\numTrainingSamplesNetzerBiop\ (median: \numTrainingSamplesBiopMedian) samples to train their deep learning system \citep{schelb2019classification, arif2020clinically, sanyal2020automated, aldoj2020semi, bhattacharya2020corrsignet, cao2019joint, seetharaman2021automated, netzer2021fully}. 
Approaches using radiologically-estimated annotations used \numTrainingSamplesSanford -\numTrainingSamplesSaha\ (median: \numTrainingSamplesRadiolMedian) training samples \citep{sanford2020deep, yu2020deep, yu2020false, saha2021end}. 

Between these two types of annotations there are important trade-offs. Histopathological annotations provide high quality ground-truth annotations \citep{radtke2016multiparametric}, but also inherently considers intermediate to high risk patients, has risk associated with acquisition \citep{loeb2011complications} and is expensive \citep{altok2018cost}. Alternatively, the less accurate radiologically-estimated ground truth (reported using Prostate Imaging Reporting and Data System: Version 2 (PI-RADS)) can be used. These annotations allow the inclusion of all patients who received an MRI examination and covers the complete distribution of patients encountered in clinical practice. It is unclear how the benefits of a wider training cohort and larger training size compare against the downside of more noise in the training annotations. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduce need for many labelled training samples %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Prior work investigated the effect of training set size on prostate cancer detection performance, with radiologically-estimated ground truth for training and testing \citep{hosseinzadeh21deep}. This work shows patient-based area under the receiver operating characteristic curve (AUROC) for their internal test set increased logarithmically between \numTrainingCasesHosseinzadehStart\ and \numTrainingCasesHosseinzadehEnd\ training cases, from an AUROC of \RUMCAUCHosseinzadehStart\ to \RUMCAUCHosseinzadehEnd. If this trend continues, it requires tens of thousands of annotated cases to reach expert performance, which is in concordance with related fields. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Automatic labelling - general %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Manually labelling training samples is a time consuming and expensive process. Trained students supervised by experienced prostate radiologists annotated the PI-RADS $\geq 4$ findings in more than three thousand of our institutional prostate MRI studies. According to our main annotator, she requires about eight minutes to annotate a single prostate cancer lesion in 3D. Difficult cases are discussed with radiologists, further increasing the overall time investment. 
Annotating tens of thousands of cases therefore would incur huge costs and an incredibly large time investment. 

Annotation time and cost is a limiting factor in many deep learning fields, making techniques that leverage unlabelled samples essential to improve performance. 
In the natural image domain, leveraging samples without target task annotations has proven to be effective, even when manually labelled samples are abundant. 
On ImageNet, with 1.3 million manually labelled training samples, all eight leaderboard holders of the past three years used additional training samples with automatically generated labels. 
Several approaches were employed, \citep{mahajan2018exploring} used 3.5 billion images from Instagram to pre-train their models by predicting the corresponding hashtag (\textit{transfer learning}); \citep{xie2020self} used a \textit{teacher} model to predict 300 million images scraped from the web and selected 130 million samples to train a new \textit{student} model (\textit{self-training}); and in \citep{pham2020meta} the teacher-student approach was pushed further by continuously updating the teacher model with reinforcement learning. 
The other five leaderboard holders focused on different research, but did incorporate automatic labelling techniques to reach state-of-the-art performance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Automatic labelling - medical imaging - general approaches %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the medical domain, popular techniques to leverage unlabelled samples include transfer learning from a distant or related task, and self-training with automatically generated labels \citep{cheplygina2019not}. 
Other techniques to leverage unlabelled samples include contrastive learning \citep{chaitanya2020contrastive, sowrirajan2021moco, azizi2021big} and self-supervised representation learning \citep{zhou2019models}. These techniques either pre-train without labels, or use model prediction as true label. 

Some approaches go beyond annotating samples using model predictions only. 
In \citep{bulten2019epithelium} they generated pixel-level epithelium cell annotations for hematoxylin and eosin (H\&E) stained prostate biopsies. After scanning the H\&E stained biopsy, they washed out the slice and treated it with an immunohistochemistry stain. This immunohistochemistry stain highlights the epithelium cells, facilitating precise automatic segmentation. These segmentation masks were subsequently translated to the H\&E stained biopsy, by co-registering the scans. These steps allowed large scale generation of epithelium annotation in H\&E stained biopsies, which would have been impossible to obtain manually. 

In \citep{bulten2019automated} they generated pixel-level Gleason score annotations in H\&E stained prostate biopsies. First, they generated precise cancer masks. Then, they extracted the Gleason scores from the pathology reports to classify the cancer masks into Gleason grades. These steps allowed the generation of Gleason score annotations in thousands of prostate biopsies, which would have been infeasible to obtain manually. 

% Ilse:
% Tijdens het werk heb ik allerlei schermen open staan, waardoor ik snel kan schakelen. Inmiddels gaan dingen ook gewoon vlot door het veel routinematig handelen. 
% 1. Navigeren naar en openen van de scans, en het rapport er bij pakken: Zeg een minuut, misschien een keer iets meer voor openen van de scans en zoeken van rapport
% 2. Het rapport lezen en de laesies lokaliseren in de scan: Dat verschilt enorm. Wanneer rapport en ProCAD niet overeenkomen dan komt er al denkwerk aan te pas. Wanneer geen puntannotatie is gegeven, of er tussen de annotatie en rapport tegenstrijdige informatie is etc dan moet ik er echt zelf over gaan oordelen  en dan kan het zijn dat ik er zo'n 10/15 minuutjes over doe.
% 3. Het vervolgens intekenen van de laesies: als de lesie is gevonden dan gaat dit vlug, zeg een minuut voor de kleine lesies, en misschien 3 minuut per lesies voor de grotere en onduidelijkere.
% ===> approx. 1 + 5 + 2 = 8 min for positive case. For negative case approx. 1 min? Gives 70% * 1 + 30% * 8 = approx. 3 min / case. 
% Consulting experts for difficult cases significantly increases the time, so ~5 min / case on average?

%%%%%%%%%%%%%%%%%%%%%%%
% % Our contributions %
%%%%%%%%%%%%%%%%%%%%%%%
In this work, we investigate automatically annotating clinically significant prostate cancer in MRI. 
Similar to \citep{bulten2019automated}, we generate annotations for unlabelled samples using model predictions, guided by information from the reports. 
First, we train a prostate cancer detection model on manually annotated visits, 
and generate lesion candidates for the unlabelled visits. Then, we count the number of clinically significant findings (PI-RADS $\geq 4$ lesions) described in the radiology report. 
Subsequently, we match the lesion candidates to the PI-RADS scores from the report, by matching the most confident lesion candidates to the highest scores. Lesion candidates matched to a PI-RADS $\geq 4$ lesion are saved as csPCa annotation. 

Our automatic labelling procedure enables us to leverage the largest dataset of MRI scans for prostate cancer detection reported in literature to date. 
We demonstrate the efficacy of our automatically generated annotations by training a prostate cancer detection model jointly on manual and automatic annotations, which significantly outperforms training on manual annotations exclusively. 

==> chapters/deprecated/2e-augmenting-PCa-segmentation.tex <==

The steps used to generate \frameworkName\ are summarised in Algorithm \ref{algo:AVA}. We use two independent prostate cancer detection architectures to demonstrate the generality of our framework. Specifically, institutional \nameUNetagpp, and the self-configuring \namennUNet\ framework. See \Cref{sec:model} for details on the model architectures, and \Cref{sec:preprocessing_training_augmentation} for details on preprocessing, training and data augmentation. \\



\begin{algorithm}[h]
\SetAlgoLined
    \textbf{Step 1}: train model on manual voxel annotations\;
    \textbf{Step 2}: predict (unlabelled) cases\;
    \textbf{Step 3}: split voxel-level predictions into predictions for distinct lesions\;
    \textbf{Step 4}: parse radiology report and count csPCa lesions\;
    \textbf{Step 4 (alternative)}: parse pathology report\;
    \textbf{Step 5}: mask lesion predictions with n/o csPCa lesions\;
    \textbf{Step 6}: scale csPCa lesion predictions\;
    \caption{\frameworkName}
    \label{algo:AVA}
\end{algorithm}



==> chapters/deprecated/2e-prep-train-augment.tex <==
\subsection{Preprocessing, Training and Data Augmentation}
\label{sec:preprocessing_training_augmentation}
% Preprocessing
The used bpMRI protocols ensures negligible patient movement between imaging sequences, and little deviation of the prostate from the centre of the scans. Therefore, no alignment was needed within a bpMRI study, or between different studies. In previous work we have experienced that a centre crop size of $(72.0, 72.0, 64.8)$ mm at a resampled resolution of $(0.5, 0.5, 3.6)$ mm/voxel works well for our dataset \citep{saha2021end}. \\

% ADC is divided by 3000, which is the 97.37026255th percentile (all 7,756 samples)
For the \nameUNetagpp\ model we have used a custom augmentation pipeline. To prevent border interpolation errors, we start with a centre crop of $(96.0, 96.0, 64.8)$ mm prior to applying augmentations. Then, we perform instance-wise min/max normalisation for T2-weighted scans and high b-value scans. For ADC scans, we divide each scan by 3000 ($97.5^{\text{th}}$ percentile), to retain their diagnostically relevant absolute values. Subsequently, with a probability of $75\%$ we apply Rician noise \citep{gudbjartsson1995rician} with $\sigma = 0.01$ to each scan at original resolution. Then, we rescale all scans to a uniform resolution of $0.5\times0.5\times3.6$ mm/voxel with bicubic interpolation. Then, with a probability of $50\%$, we apply 2D affine data augmentations: horizontal mirroring, rotation with $\theta \sim 7.5\cdot\mathcal{N}(0, 1)$, horizontal translation with $h_x \sim 0.05\cdot\mathcal{N}(0, 1)$, vertical translation with $h_y \sim 0.05\cdot\mathcal{N}(0, 1)$ and zoom with $s_{xy} \sim 1.05\cdot\mathcal{N}(0, 1)$, where $\mathcal{N}(0, 1)$ is a Gaussian distribution with zero mean and unit variance. Finally, we centre crop to $(72.0, 72.0, 64.8)$ mm. \\

% Training
Based on prior experience \citep{saha2021end}, we trained the \nameUNetagpp\ model with Focal Loss ($\alpha=0.75$) \citep{lin2017focal}. \\

The \namennUNet\ framework uses the unweighted sum of cross-entropy and soft Dice loss, and applies the loss at multiple resolutions (deep supervision). % For our task, the \namennUNet configured itself to use  At each stage, a downsampled version of the ground truth segmentation map is used to compute the loss, 
% and configured itself to apply the loss at the four highest resolution stages. At  The losses are calculated at the four highest resolution stages, with weights halv. 
Based on prior work \citep{saha2021end} we have resampled all bpMRI scans to a uniform spacing of $(0.5, 0.5, 3.6)$ mm/voxel. We performed a slightly larger centre crop of $(80.0, 80.0, 72.0)$ mm to create inputs of $(160, 160, 20)$ voxels, which is compatible with \namennUNet\ without padding. \\

% Data augmentation
\namennUNet\ uses similar data augmentations as our custom augentation pipeline. Specifically, they apply affine transformations in 2D with a per-augmentation probability of $20\%$: mirroring over all three axes, rotation with $\theta \sim \mathcal{U}(-\pi, \pi)$ horizontal translation with $h_x \sim 0.05\cdot\mathcal{N}(0, 1)$, vertical translation with $h_y \sim 0.05\cdot\mathcal{N}(0, 1)$ and zoom with $s \sim \mathcal{U}(0.7, 1.4)$

% \input{chapters/2d-augmentation-details}
% Augmentations:
% 'do_gamma': True, 'gamma_retain_stats': True, 'gamma_range': (0.7, 1.5), 'p_gamma': 0.3, 


%  ===> See https://www.nature.com/articles/s41592-020-01008-z --> Training schedule
% From /mnt/netcache/pelvis/projects/joeran/Data/nnUNet_raw_data_base/results/nnUNet/3d_fullres/Task101_Prostate_mpMRI_csPCa/nnUNetTrainerV2__nnUNetPlansv2.1/plans.pkl:

% Architecture:
%   'current_spacing': array([3.5999999, 0.5      , 0.5      ]),
%   'original_spacing': array([3.5999999, 0.5      , 0.5      ]),
%   'do_dummy_2D_data_aug': True,
%   'pool_op_kernel_sizes': [[1, 2, 2],
%     [1, 2, 2],
%     [2, 2, 2],
%     [2, 2, 2],
%     [1, 2, 2]],
%   'conv_kernel_sizes': [[1, 3, 3],
%     [1, 3, 3],
%     [3, 3, 3],
%     [3, 3, 3],
%     [3, 3, 3],
%     [3, 3, 3]]}},
%  'conv_per_stage': 2}


% "ds_loss_weights": "[0.53333333 0.26666667 0.13333333 0.06666667 0.        ]"

%  Training:
% batch_size = 7, 
% num_pool_per_axis = [2, 5, 5],
% patch_size = [ 20, 160, 160], 
% median_patient_size_in_voxels: [ 18, 144, 144],
%  "initial_lr": "0.01",
%  "lr_scheduler_eps": "0.001",
%  "lr_scheduler_patience": "30",
%  "lr_threshold": "1e-06",
%  "max_num_epochs": "1000",
%  "num_batches_per_epoch": "250",
%  "optimizer": "SGD (\nParameter Group 0\n    dampening: 0\n    lr: 0.01\n    momentum: 0.99\n    nesterov: True\n    weight_decay: 3e-05\n)",
%  "oversample_foreground_percent": "0.33",

% Augmentations:
% 'do_gamma': True, 'gamma_retain_stats': True, 'gamma_range': (0.7, 1.5), 'p_gamma': 0.3, 'do_mirror': True, 'mirror_axes': (0, 1, 2), 'dummy_2D': True, 
%  'do_scaling': True, 'scale_range': (0.7, 1.4), 'p_scale': 0.2, 'do_rotation': True, 'rotation_x': (-3.141592653589793, 3.141592653589793), 'rotation_y': (-0.5235987755982988, 0.5235987755982988), 'rotation_z': (-0.5235987755982988, 0.5235987755982988), 'rotation_p_per_axis': 1, 'p_rot': 0.2,


==> chapters/deprecated/2f-augmentation-details.tex <==
\begin{table*}[!t]
\caption{\label{tab1}Data augmentations used during model training}
\centering
\begin{tabular}{l|ll|ll}
\toprule
Model                                               & \multicolumn{2}{c|}{\nameUNetagpp}  & \multicolumn{2}{c}{\namennUNet}                                                                                     \\ \hline
Normalisation                                              & \multicolumn{2}{l|}{(Instance-wise) min/max}           & \multicolumn{2}{l}{(Instance-wise) zero mean, unit variance}                                                                                                     \\ \hline
Augmentation                                               &  Distribution                                  & Probability       & Distribution                                         & Probability       \\ \hline
Mirror                                                     & Horizontal           & $50\%$ shared     & All axes                                                                                            & $50\%$ individual \\
Rotation (degrees)                                         & $7.5\cdot\mathcal{N}(0, 1)$   & $50\%$ shared     & $\mathcal{U}(-180, 180)$                                                                       & $20\%$ individual \\
Zoom (affine scaling factor)                               & $1.05\cdot\mathcal{N}(0, 1)$  & $50\%$ shared     & $\mathcal{U}(0.7, 1.4)$                                                                        & $20\%$ individual \\
Translation, horizontal                                    & $0.05 \cdot\mathcal{N}(0, 1)$ & $50\%$ shared     & -                                                                                                   & -                 \\
Translation, vertical                                      & $0.05 \cdot\mathcal{N}(0, 1)$ & $50\%$ shared     & -                                                                                                   & -                 \\
Additive noise                                       & $\text{Rician}(\sigma=0.01)$         & $75\%$ individual & $\mathcal{N}(0, \sigma)$, with $\sigma \sim \mathcal{U}(0, 0.1)$                               & $15\%$ individual \\
Gaussian blur                                              & -                                  & -                 & See \citep{isensee2021nnu}, Sup. Mat. Note 4                                 & $20\%$ individual \\
Brightness                                           & -                                  & -                 & $\mathcal{U}(0.7, 1.3)$                                                                        & $15\%$ individual \\
Contrast                                                   & -                                  & -                 & $\mathcal{U}(0.65, 1.5)$, with subsequent clipping & $15\%$ individual \\
Simulation of low resolution                               & -                                  & -                 & See \citep{isensee2021nnu}, Sup. Mat. Note 4                                 & $25\%$ individual \\
Gamma augmentation                                         & -                                  & -                 & See \citep{isensee2021nnu}, Sup. Mat. Note 4                                 & $15\%$ individual
\end{tabular}
\end{table*}

==> chapters/deprecated/outline.tex <==


=== Introduction ===
- Prevalence of PCa 
--> Need for risk stratification and lesions detection
- Manual voxel annotations are expensive
- Related work
--> Related works use either low number of biopsy-confirmed PCa, or medium number of radiology-estimated PCa
- Our contributions
--> We introduce automatic voxel annotation of report findings
--> Using our AVA, we pushed the number of radiology-estimated PCa training samples to 3x that of prior arts and the number of biopsy-confirmed PCa training samples to 5x that of prior arts


=== Materials and Methods ===
- Heterogeneous dataset
--> 9k visits with radiology report from clinical routine
--> 3k manual csPCa annotations
--> 2k pathology reports from clinical routine

- Automatic finding extraction from reports
--> Used to determine number of csPCa lesions
--> Rule-based NLP script
--> 1. split report in sections for each lesion (91\%)
--> 2. extract T2, ADC and DCE and total scores
--> 3. count number of lesions with PI-RADS >= 4

- Automatic Voxel Annotation:
--> Train model on expert csPCa segmentations
--> Propose candidates
--> Mask csPCa candidates with n/o csPCa lesions
--> Scale soft masks to match manual segmentations
--> Apply 3D Gaussian smoothing to manual segmentations to harmonise labels

- Deep Learning Detection Model
--> 3D UNet with attention stuff
--> Detection model same as in Saha2021, but with LeakyReLU in decoder
--> nnUNet
--> Preprocessing, training and data augmentation
    --> Focal loss (alpha=0.75) for M1, binary Gaussian smoothing for labels
    --> Center crop to [96.0, 96.0, 64.8] mm
    --> Instance-wise min/max normalisation for T2W & DWI, /3000 for ADC
    --> Rician noise at original resolution, p=0.75, sigma=0.01
    --> Rescale to 0.5 x 0.5 x 3.6 mm/voxel
    --> Augmentations with prob=50\%: horizontal mirroring ~ U{yes, no}, rotate degrees ~ 7.5*N(0, 1), translate with 0.05 * N(0, 1), zoom with 1.05 * N(0, 1)
    --> Center crop to [72.0, 72.0, 64.8] mm

- Zonal segmentation/prior?


=== Results ===
- Automatic segmentation performance (AUROC/FROC of soft pseudo labels, both for masking with radiology reports and pathology reports). Best to do on RUMC to indicate that the report-algorithm doesn't necessarily generalise?
- Experiment 1: as in RSNA, but with LeakyReLU, more samples and scaled pseudo labels
- Experiment 2: exp 3 from TRAC; biopsy only vs radiology only vs hybrid

=== Conclusion ===

=== Discussion ===

=== Acknowledgements ===


==> figures/AVA-quality-DSC.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{figures/pdfs/AVA_DSC_distribution_vertical_unfiltered.pdf}
    \caption{Spatial congruence between automatic and manual csPCa annotations, as measured by the Dice similarity coefficient, for automatic annotations derived from \ieeeblue{(top)}\ \namennUNet\ or \ieeeblue{(bottom)}\ \nameUNetagpp. 
    Both methods are evaluated on the labelled \nameRUMC\ dataset with 5-fold cross-validation, exclude studies due to empty PI-RADS extraction from the radiology report, and exclude studies with insufficient lesion candidates. 
    All metrics are computed in 3D. 
    }
    \label{fig:AVA-quality-DSC}
\end{figure}

==> figures/MRI-sequences.tex <==
\begin{table}[]
\caption{Series descriptions identified for T2W, ADC and high b-value}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Sequence} & \textbf{Series description}                          & \textbf{Frequency} \\ \midrule
T2W axial         & t2\_tse\_tra                                         & 9214                 \\
                  & t2\_tse\_tra\_snel                                   & 5941                 \\
                  & t2\_tse\_tra\_snel\_bij bewogen t2 tra               & 1184                 \\ \midrule
ADC               & ep2d\_diff\_tra\_ADC\_DFC                            & 8748                 \\
                  & \begin{tabular}[c]{@{}l@{}}diff tra b 50 500 800 WIP511b alle \\ spoelen\_ADC\end{tabular}      & 256                  \\
                  & ep2d\_diff\_tra\_orig\_ADC\_DFC                      & 47                   \\
                  & ep2d\_diff\_tra\_ADC                                 & 46                   \\
                  & diff tra b 50 500 800 WIP511E\_ADC                   & 32                   \\ \midrule
High b-value      & ep2d\_diff\_tra\_CALC\_BVAL\_DFC                     & 8748                 \\
                  & \begin{tabular}[c]{@{}l@{}}diff tra b 50 500 800 WIP511b alle \\ spoelenCALC\_BVAL\end{tabular} & 256                  \\
                  & ep2d\_diff\_tra\_orig\_CALC\_BVAL\_DFC               & 47                   \\
                  & ep2d\_diff\_tra\_CALC\_BVAL                          & 46                   \\
                  & diff tra b 50 500 800 WIP511ECALC\_BVAL              & 32                   \\ \midrule
T2W coronal       & t2\_tse\_cor                                         & 8747                 \\
                  & t2\_spc\_3D\_cor\_iso                                & 463                  \\ \midrule
T2W sagittal      & t2\_tse\_sag                                         & 9214                 \\ \midrule
Do NOT use        & resolve\_diff\_tra\_CALC\_BVAL                       & 248                  \\
                  & resolve\_diff\_tra\_ADC                              & 248                  \\
                  & resolve\_diff\_b50\_400\_800\_tra\_CALC\_BVAL        & 37                   \\
                  & resolve\_diff\_b50\_400\_800\_tra\_ADC               & 37                   \\ \bottomrule
\end{tabular}
\label{tab:MRI-sequences}
\end{table}

==> figures/detector_networks.tex <==
\begin{figure*}[t!]
    \centering
    % \includegraphics[width=.9\textwidth]{figures/pdfs/detector_architecture-M1.pdf}
    % \includegraphics[width=.9\textwidth]{figures/pdfs/detector_architecture-nnUNet.pdf}
    \includegraphics[width=\textwidth]{figures/pdfs/nnUNet-PCa-data.pdf}
    \caption{Architecture schematic of the \namennUNet, as configured for our prostate cancer segmentation task. }
    \label{fig:detector_networks}
\end{figure*}


==> figures/report-finding-extraction-long.tex <==

\begin{figure*}
\centering
\begin{tabular}{c|c}
    \begin{minipage}[c]{0.47\textwidth}\includegraphics[width=\textwidth]{figures/pdfs/report-finding-extraction.pdf}\vspace{\abovecaptionskip}\end{minipage} & %
    \begin{minipage}[c]{0.47\textwidth}\input{figures/report_text/sample-1}\vspace{\belowcaptionskip}\end{minipage} \\ \hline
    
    \begin{minipage}[c]{0.47\textwidth}\vspace{\abovecaptionskip}\input{figures/report_text/sample-2}\vspace{\belowcaptionskip}\end{minipage} & %
    \begin{minipage}[c]{0.47\textwidth}\vspace{\abovecaptionskip}\input{figures/report_text/sample-3}\vspace{\belowcaptionskip}\end{minipage}
\end{tabular}
\caption{Automatic extraction of report findings from radiology reports. (top left panel) schematic depiction of the steps to extract PI-RADS scores: 1. split the report in sections per lesion and 2. extract the PI-RADS score and individual T2/DWI/DCe scores for each lesion. (top right and bottom left panels) typical report snippets of clinically significant lesions, with the extracted scores coloured in. The reports are divided in section by matching the patterns \color{C0}Index lesion mark1\color{black}\ and \color{C0}Finding nr. 1\color{black}. (bottom right panel) Example of a case where simple extraction of PI-RADS scores would fail, indicating the benefit of a more sophisticated pattern matching.  }
\label{fig:finding_extraction_radiology_report}
\end{figure*}


==> figures/table-related-work-samples.tex <==
\begin{table*}[!t]
\caption{\label{tab1}Number of samples used for training}
\centering
\begin{tabular}{lrll}%{|p{2.25cm}|p{2cm}|l|p{4cm}|p{3cm}|p{2cm}|}
\toprule
\textbf{Study}                     & \textbf{Training samples}          & \textbf{Ground thruth}    & \textbf{\begin{tabular}[c]{@{}l@{}}Estimated error rate \\ (patient level, relative to WMHP)\end{tabular}  }              \\ \midrule
\citep{schelb2019classification}   & \numTrainingSamplesSchelb\         & MRI-GB + TRUS      & $3\%$ \citep{radtke2016multiparametric}                            \\ \midrule
\citep{sanford2020deep}            & \numTrainingSamplesSanford\        & PI-RADS            & $24\%$ (rough estimate, refine if used) \\ \midrule
\citep{arif2020clinically}         & \numTrainingSamplesArif\           & MRI-GB + TRUS   &  \\ \midrule % additionally they use PI-RADS to decide if samples should be excluded (21 / 292 = 7% is excluded)
\citep{yu2020deep}                 & \numTrainingSamplesYuDetection\    & PI-RADS & $24\%$ (rough estimate, refine if used) \\ \midrule
\citep{yu2020false}                & \numTrainingSamplesYuFPReduction\  & PI-RADS & $24\%$ (rough estimate, refine if used) \\ \midrule
\citep{sanyal2020automated}        & \numTrainingSamplesSanyal\         & Pathology, not further specified & $\approx 3\%$ \\ \midrule
\citep{aldoj2020semi}              & \numTrainingSamplesAldroj\         & Pathology, not further specified & $\approx 3\%$ \\ \midrule
\citep{bhattacharya2020corrsignet} & \numTrainingSamplesBhattacharya\   & WMHP               & - \\ \midrule
\citep{cao2021performance}         & \numTrainingSamplesCao\            & WMHP               & -    \\ \midrule
\citep{seetharaman2021automated}   & \numTrainingSamplesSeetharaman\    & WMHP or biopsy     & $\leq 3\%$    \\ \midrule
\citep{saha2021end}                & \numTrainingSamplesSaha\           & PI-RADS            & $24\%$ (rough estimate, refine if used)   \\ \midrule
Proposed radiology-only approach   & \numTrainingSamplesProposedPIRADS\ & PI-RADS            & 24\% (rough estimate, refine if used)                                                          \\ \midrule
Proposed biopsy-only approach      & \numTrainingSamplesProposedBiopsy\ & MRI-GB + TRUS      & 3\% \citep{radtke2016multiparametric}     \\ \midrule
Proposed hybrid approach           & \numTrainingSamplesProposedHybrid\ & \begin{tabular}[c]{@{}l@{}}MRI-GB + TRUS, \\ or PI-RADS\end{tabular} & \begin{tabular}[c]{@{}l@{}}$4\%$ (rough estimate, refine if used. \\ Weighed average of $3\%$ for \numTrainingSamplesProposedBiopsy\ \\ samples and $5\%$ for \numTrainingSamplesProposedHybridnumPIRADS) \end{tabular} \\ \bottomrule
\end{tabular}
\end{table*}


==> figures/table-treatments.tex <==
\begin{table}[]
\caption{Excluded treatments}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Previously matched treatments}      & \textbf{Additional treatments} &  \\ \midrule
RALP                                        & TUR                            &  \\
Robotic-assisted laparoscopic prostatectomy & laser focale                   &  \\
laparoscopic                                & TULSA                          &  \\
radiotherapie                               & prostectomie                   &  \\
radiation                                   & focale behandeling             &  \\
radiotherapy                                & MRI laser behandeling          &  \\
HIFU                                        & bestraling                     &  \\
prostectomy                                 & hemi-ablatie                   &  \\
TURP                                        & ablatie                        &  \\
resection                                   & laserablatie                   &  \\
cryo                                        & anteriorresectie               &  \\
prostatectomie                              & sigmoidresectie                &  \\
brachytherapie                              & Green light laser              &  \\
therapie                                    & TURT                           &  \\
resectie                                    & chemotherapie                  &  \\
RRP                                         & LHRH                           &  \\
radicale prostatectomy                      &                                &  \\
prostatectomy                               &                                &  \\
EBRT                                        &                                &  \\
radiation therapy                           &                                &  \\
chemoradiatie                               &                                &  \\
na de chirurgie                             &                                &  \\
chirurgie                                   &                                &  \\
Hormonen                                    &                                &  \\
TURS                                        &                                &  \\ \bottomrule
\end{tabular}
\label{tab:excluded-treatments}
\end{table}
